Automatic Calibration for Membership Inference Attack on Large Language Models

Membership Inference Attacks (MIAs) have recently been employed to determine whether a specific text was part of the pre-training data of Large Language Models (LLMs). However, existing methods often misinfer non-members as members, leading to a high false positive rate, or depend on additional reference models for probability calibration, which limits their practicality. To overcome these challenges, we introduce a novel framework called Automatic Calibration Membership Inference Attack (ACMIA), which utilizes a tunable temperature to calibrate output probabilities effectively. This approach is inspired by our theoretical insights into maximum likelihood estimation during the pre-training of LLMs. We introduce ACMIA in three configurations designed to accommodate different levels of model access and increase the probability gap between members and non-members, improving the reliability and robustness of membership inference. Extensive experiments on various open-source LLMs demonstrate that our proposed attack is highly effective, robust, and generalizable, surpassing state-of-the-art baselines across three widely used benchmarks. Our code is available at: \href{https://github.com/Salehzz/ACMIA}{\textcolor{blue}{Github}}.

==> tables/ablation.tex <==
\begin{table}[t]
\centering
\caption{AUROC results for ARMIA with different calibration methods on Pythia-12B, averaged across all MIMIR datasets and WIKIMIA lengths, including original and paraphrased settings.}
\label{tab:ablation}
\begin{tabular}{ccccc}
\toprule
Method  & WikiMIA & MIMIR \\ \midrule
Temperature & 67.1 & 64.2 \\
NormAR & \textbf{70.5} & 65.2 \\
AR & 70.1 & \textbf{65.8} \\
\bottomrule
\end{tabular}
\vspace{-0.3cm}
\end{table}


==> tables/mimir_auroc.tex <==
\begin{table*}[b]
\caption{AUROC results on the challenging MIMIR benchmark \cite{mimir} with a suite of Pythia models \cite{pythia}. In each column, the best result across all methods is \textbf{bolded}, with the runner-up \underline{underlined}. 
$^\dag$Ref relies on a reference LLM.
$^\ddag$Neighbor induces significant extra computational cost than others ($25\times$ in this case), for which reason we don't run on the 12B model. Despite not requiring a reference model like the Ref method does, our methods consistently achieve superior or comparable performance.\\
13-0.8
}
\label{tab:mimir_auroc}
\begin{center} \scriptsize
\setlength{\tabcolsep}{0.7pt}
\begin{tabularx}{\textwidth}{l *{20}{>{\centering\arraybackslash}X}@{}}
    \toprule
    \multirow{2}{*}{}  & \multicolumn{5}{c}{\textbf{Wikipedia}} & \multicolumn{5}{c}{\textbf{Github}} & \multicolumn{5}{c}{\textbf{Pile CC}} & \multicolumn{5}{c}{\textbf{PubMed Central}} \\
    \cmidrule(lr){2-6}  \cmidrule(lr){7-11} \cmidrule(lr){12-16} \cmidrule(lr){17-21}
    \textbf{Method}
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    \\
    \midrule
    
Loss \cite{yeom2018privacy}
& 50.2 & 51.3 & 51.8 & 52.8 & 53.3 & 65.7 & 69.8 & 71.3 & 73.0 & 73.9 & 49.6 & 50.0 & 50.1 & 50.7 & 51.0 & 49.9 & 49.8 & 49.9 & 50.6 & 51.2
\\
$^\dag$Ref \cite{carlini2021extracting}
& 51.2 & 55.2 & 58.1 & 61.8 & 63.0 & 64.0 & 67.1 & 65.4 & 64.4 & 63.9 & 49.2 & 52.2 & 53.7 & 54.9 & 56.7 & 51.3 & 53.1 & 53.7 & 55.9 & 58.0
\\
Lowercase \cite{carlini2021extracting}
& 50.1 & 51.3 & 51.7 & 53.5 & 53.8 & 67.2 & 70.3 & 71.3 & 72.9 & 73.6 & 47.8 & 48.6 & 49.5 & 50.1 & 50.4 & 49.5 & 50.4 & 51.5 & 51.5 & 52.6
\\
Zlib \cite{carlini2021extracting}
& 51.1 & 52.0 & 52.4 & 53.5 & 54.1 & 67.5 & 71.0 & 72.3 & 73.9 & 74.7 & 49.6 & 50.1 & 50.3 & 50.8 & 51.1 & 49.9 & 50.0 & 50.1 & 50.6 & 51.0
\\
$^\ddag$Neighbor \cite{mia_neighbor}
& 50.7 & 51.7 & 52.2 & 53.2 & / & 65.3 & 69.4 & 70.5 & 72.1 & / & 49.6 & 50.0 & 50.1 & 50.8 & / & 47.9 & 49.1 & 49.7 & 50.1 & /
\\
Min-K\% \cite{shi2023detecting}
& 50.2 & 51.3 & 51.8 & 53.6 & 54.2 & 65.7 & 69.9 & 71.4 & 73.2 & 74.2 & 50.3 & 51.0 & 50.8 & 51.5 & 51.6 & 50.6 & 50.3 & 50.5 & 51.2 & 52.1
\\
Min-K\%++ \cite{zhang2024min}
& 49.7 & 53.7 & 55.1 & 58.0 & 59.9 & 64.8 & 69.6 & 70.9 & 72.8 & 73.7 & 50.6 & 51.0 & 51.0 & 53.0 & 53.0 & 50.6 & 51.4 & 52.4 & 54.2 & 55.0
\\
Normalized Temp
& 50.9 & 53.6 & 55.1 & 58.0 & 59.9 & 65.8 & 69.1 & 70.1 & 72.1 & 72.9 & 52.1 & 51.8 & 52.0 & 53.4 & 53.3 & 51.1 & 51.7 & 52.5 & 54.2 & 55.0
\\
Temp - Original
& 50.3 & 52.9 & 54.1 & 57.1 & 59.1 & 66.0 & 70.0 & 71.6 & 73.6 & 74.4 & 51.8 & 52.5 & 52.6 & 54.1 & 54.0 & 50.9 & 51.7 & 52.9 & 54.4 & 55.2
\\

        \vspace{-.6em} \\
    
    \toprule
    \multirow{2}{*}{}  & \multicolumn{5}{c}{\textbf{ArXiv}} & \multicolumn{5}{c}{\textbf{DM Mathematics}} & \multicolumn{5}{c}{\textbf{HackerNews}} & \multicolumn{5}{c}{\textbf{Average}}\\
    \cmidrule(lr){2-6}  \cmidrule(lr){7-11} \cmidrule(lr){12-16} \cmidrule(lr){17-21}
    \textbf{Method} 
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    \\
    \midrule

Loss \cite{yeom2018privacy} 
& 51.0 & 51.5 & 51.9 & 52.9 & 53.3 & 48.8 & 48.5 & 48.4 & 48.5 & 48.5 & 49.4 & 50.5 & 51.3 & 52.1 & 52.6 & 52.1 & 53.1 & 53.5 & 54.4 & 54.8
\\
$^\dag$Ref \cite{carlini2021extracting} 
& 49.4 & 51.5 & 53.1 & 55.8 & 57.1 & 51.1 & 51.1 & 50.5 & 51.1 & 50.9 & 49.1 & 52.2 & 55.1 & 57.9 & 59.6 & 52.2 & 54.6 & 55.7 & 57.4 & 58.5
\\
Lowercase \cite{carlini2021extracting}
& 50.8 & 50.7 & 51.3 & 51.9 & 52.3 & 48.9 & 49.0 & 49.0 & 49.1 & 48.1 & 49.0 & 50.4 & 51.1 & 51.6 & 52.1 & 51.9 & 53.0 & 53.6 & 54.4 & 54.7
\\
Zlib \cite{carlini2021extracting}
& 50.1 & 50.9 & 51.3 & 52.2 & 52.5 & 48.1 & 48.2 & 48.0 & 48.1 & 48.0 & 49.7 & 50.3 & 50.8 & 51.2 & 51.5 & 52.3 & 53.2 & 53.6 & 54.3 & 54.7
\\
$^\ddag$Neighbor \cite{mia_neighbor} 
& 50.7 & 51.4 & 51.8 & 52.2 & / & 49.0 & 47.0 & 46.8 & 46.6 & / & 50.9 & 51.7 & 51.5 & 51.9 & / & 52.0 & 52.9 & 53.2 & 53.8 & /
\\
Min-K\% \cite{shi2023detecting}
& 51.0 & 51.7 & 52.5 & 53.6 & 54.4 & 49.4 & 49.7 & 49.5 & 49.6 & 49.7 & 50.9 & 51.3 & 52.6 & 53.6 & 54.5 & 52.6 & 53.6 & 54.2 & 55.2 & 55.8
\\
Min-K\%++ \cite{zhang2024min}
& 50.1 & 51.1 & 53.7 & 55.2 & 57.6 & 50.5 & 50.9 & 51.7 & 51.6 & 52.0 & 50.7 & 51.3 & 52.6 & 54.5 & 56.3 & 52.4 & 54.1 & 55.3 & 57.0 & 58.2
\\
Normalized Temp
& 50.9 & 51.6 & 54.4 & 55.6 & 57.6 & 51.8 & 52.3 & 52.8 & 53.5 & 52.4 & 51.1 & 50.7 & 52.5 & 54.3 & 56.3 & 53.4 & 54.4 & 55.6 & 57.3 & 58.2
\\
Temp - Original
& 51.4 & 51.7 & 53.9 & 55.8 & 57.4 & 51.6 & 51.7 & 51.9 & 52.0 & 52.2 & 49.9 & 50.5 & 52.1 & 53.9 & 55.8 & 53.1 & 54.4 & 55.6 & 57.3 & 58.3
\\
    
    \bottomrule
\end{tabularx}
\end{center}
% \vskip -0.1in
\end{table*}

==> tables/mimir_auroc_13_0.2.tex <==
\begin{table*}[b]
\caption{AUROC results on the challenging MIMIR benchmark \cite{mimir} with a suite of Pythia models \cite{pythia}. In each column, the best result across all methods is \textbf{bolded}, with the runner-up \underline{underlined}. 
$^\dag$Ref relies on a reference LLM.
$^\ddag$Neighbor induces significant extra computational cost than others ($25\times$ in this case), for which reason we don't run on the 12B model. Despite not requiring a reference model like the Ref method does, our \method{} consistently achieves superior or comparable performance.\\
13-0.2
}
\label{tab:mimir_auroc}
\begin{center} \scriptsize
\setlength{\tabcolsep}{0.7pt}
\begin{tabularx}{\textwidth}{l *{20}{>{\centering\arraybackslash}X}@{}}
    \toprule
    \multirow{2}{*}{}  & \multicolumn{5}{c}{\textbf{Wikipedia}} & \multicolumn{5}{c}{\textbf{Github}} & \multicolumn{5}{c}{\textbf{Pile CC}} & \multicolumn{5}{c}{\textbf{PubMed Central}} \\
    \cmidrule(lr){2-6}  \cmidrule(lr){7-11} \cmidrule(lr){12-16} \cmidrule(lr){17-21}
    \textbf{Method}
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    \\
    \midrule
    
Loss \cite{yeom2018privacy}
& 51.2 & 53.4 & 54.1 & 55.6 & 56.3 & 76.3 & 80.2 & 81.4 & 82.7 & 83.5 & 50.1 & 51.0 & 51.2 & 52.1 & 52.6 & 50.9 & 52.1 & 52.7 & 53.4 & 53.8
\\
$^\dag$Ref \cite{carlini2021extracting}
& 50.2 & 57.1 & 59.9 & 65.1 & 66.7 & 70.5 & 74.6 & 71.6 & 70.2 & 69.5 & 50.5 & 55.0 & 56.3 & 58.7 & 60.3 & 48.9 & 54.1 & 56.1 & 58.6 & 59.4
\\
Lowercase \cite{carlini2021extracting}
& 50.9 & 53.9 & 54.4 & 56.4 & 56.9 & 79.8 & 81.6 & 82.4 & 83.8 & 84.4 & 50.6 & 51.5 & 52.3 & 53.3 & 54.5 & 52.2 & 54.1 & 54.6 & 55.3 & 55.4
\\
Zlib \cite{carlini2021extracting}
& 50.4 & 53.1 & 54.0 & 55.7 & 56.5 & 79.7 & 82.9 & 83.9 & 85.0 & 85.7 & 51.1 & 52.1 & 52.3 & 53.2 & 53.5 & 51.5 & 52.6 & 53.1 & 53.7 & 54.0
\\
Min-K\% \cite{shi2023detecting}
& 51.2 & 53.6 & 54.7 & 57.0 & 57.8 & 76.3 & 80.2 & 81.4 & 82.8 & 83.5 & 50.9 & 51.8 & 52.3 & 53.0 & 53.2 & 51.4 & 52.6 & 53.0 & 53.9 & 54.6
\\
Min-K\%++ \cite{zhang2024min}
& 51.7 & 55.4 & 57.0 & 60.4 & 61.7 & 73.7 & 78.4 & 79.8 & 81.2 & 82.1 & 51.5 & 53.5 & 53.2 & 54.9 & 55.3 & 50.7 & 52.7 & 53.4 & 55.2 & 55.4
\\
Normalized Temp
& 52.1 & 55.1 & 56.6 & 60.0 & 61.4 & 77.2 & 78.3 & 79.7 & 81.3 & 82.2 & 51.5 & 53.5 & 53.1 & 54.8 & 55.3 & 51.4 & 52.6 & 53.4 & 54.9 & 55.2
\\
Temp - Original
& 52.0 & 55.0 & 56.3 & 59.7 & 61.4 & 76.1 & 80.0 & 81.3 & 82.7 & 83.5 & 51.6 & 54.1 & 53.5 & 55.1 & 55.3 & 51.0 & 52.8 & 53.7 & 55.4 & 56.0
\\

        \vspace{-.6em} \\
    
    \toprule
    \multirow{2}{*}{}  & \multicolumn{5}{c}{\textbf{ArXiv}} & \multicolumn{5}{c}{\textbf{DM Mathematics}} & \multicolumn{5}{c}{\textbf{HackerNews}} & \multicolumn{5}{c}{\textbf{Average}}\\
    \cmidrule(lr){2-6}  \cmidrule(lr){7-11} \cmidrule(lr){12-16} \cmidrule(lr){17-21}
    \textbf{Method} 
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    \\
    \midrule

Loss \cite{yeom2018privacy} 
& 54.6 & 55.8 & 56.4 & 57.5 & 57.8 & 67.8 & 67.5 & 67.2 & 67.3 & 67.4 & 50.5 & 51.8 & 52.6 & 53.4 & 54.0 & 57.3 & 58.8 & 59.4 & 60.3 & 60.8
\\
$^\dag$Ref \cite{carlini2021extracting} 
& 50.3 & 54.9 & 56.3 & 59.1 & 59.9 & 53.8 & 47.2 & 45.1 & 44.9 & 44.6 & 49.1 & 52.3 & 55.1 & 58.2 & 60.2 & 53.3 & 56.5 & 57.2 & 59.3 & 60.1
\\
Lowercase \cite{carlini2021extracting}
& 53.7 & 54.2 & 55.2 & 55.8 & 56.7 & 56.5 & 56.6 & 58.6 & 58.0 & 56.7 & 49.3 & 50.6 & 51.5 & 52.1 & 52.3 & 56.1 & 57.5 & 58.4 & 59.2 & 59.6
\\
Zlib \cite{carlini2021extracting}
& 54.2 & 55.3 & 55.7 & 56.7 & 57.0 & 64.6 & 64.7 & 64.6 & 64.6 & 64.6 & 51.2 & 51.9 & 52.4 & 52.9 & 53.2 & 57.5 & 58.9 & 59.4 & 60.3 & 60.6
\\
Min-K\% \cite{shi2023detecting}
& 54.6 & 55.8 & 56.4 & 57.5 & 58.2 & 67.8 & 67.5 & 67.2 & 67.3 & 67.4 & 51.2 & 52.1 & 53.4 & 54.4 & 55.1 & 57.6 & 59.1 & 59.8 & 60.8 & 61.4
\\
Min-K\%++ \cite{zhang2024min}
& 52.1 & 54.4 & 56.4 & 57.7 & 60.1 & 59.2 & 58.6 & 59.9 & 59.4 & 59.5 & 51.1 & 51.6 & 53.1 & 55.0 & 56.3 & 55.7 & 57.8 & 59.0 & 60.5 & 61.5
\\
Normalized Temp
& 54.8 & 55.7 & 56.1 & 57.2 & 59.6 & 65.5 & 65.3 & 65.1 & 65.7 & 64.7 & 51.2 & 51.7 & 53.1 & 54.8 & 56.1 & 57.7 & 58.9 & 59.6 & 61.2 & 62.1
\\
Temp - Original
& 54.6 & 56.0 & 56.9 & 58.5 & 59.8 & 67.7 & 68.5 & 68.0 & 68.4 & 68.3 & 50.7 & 51.7 & 52.8 & 54.4 & 55.9 & 57.7 & 59.7 & 60.4 & 62.0 & 62.9
\\
    
    \bottomrule
\end{tabularx}
\end{center}
% \vskip -0.1in
\end{table*}

==> tables/mimir_auroc_7_0.2.tex <==
\begin{table*}[b]
\caption{AUROC results on the challenging MIMIR benchmark \cite{mimir} with non-member sets at \le 20\% 7-gram overlap threshold with a suite of Pythia models \cite{pythia}. In each column, the best result across all methods is \textbf{bolded}, with the runner-up \underline{underlined}. 
$^\dag$Ref relies on a reference LLM.
Despite not requiring a reference model like the Ref method does, our methods consistently achieve superior or comparable performance.\\
}
\label{tab:mimir_auroc_7_2}
\begin{center} \scriptsize
\setlength{\tabcolsep}{0.7pt}
\begin{tabularx}{\textwidth}{l *{20}{>{\centering\arraybackslash}X}@{}}
    \toprule
    \multirow{2}{*}{}  & \multicolumn{5}{c}{\textbf{Wikipedia}} & \multicolumn{5}{c}{\textbf{Github}} & \multicolumn{5}{c}{\textbf{Pile CC}} & \multicolumn{5}{c}{\textbf{PubMed Central}} \\
    \cmidrule(lr){2-6}  \cmidrule(lr){7-11} \cmidrule(lr){12-16} \cmidrule(lr){17-21}
    \textbf{Method}
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    \\
    \midrule
    
Loss \cite{yeom2018privacy}
& 62.6 & 65.6 & 66.3 & 67.9 & 68.7 & 84.2 & 87.3 & 88.0 & 88.9 & 89.5 & 53.3 & 54.5 & 55.0 & 56.1 & 56.5 & 79.3 & 78.5 & 78.1 & 78.2 & 78.0
\\
$^\dag$Ref \cite{carlini2021extracting}
& 53.7 & 65.1 & 68.1 & 72.4 & 73.9 & 71.5 & 78.6 & 73.4 & 70.7 & 70.0 & 51.1 & 56.3 & 58.3 & 60.8 & 61.9 & 68.5 & 67.9 & 62.9 & 62.4 & 60.0
\\
Lowercase \cite{carlini2021extracting}
& 61.8 & 64.4 & 64.8 & 66.9 & 67.3 & 83.4 & 86.0 & 86.9 & 88.1 & 89.1 & 50.5 & 53.5 & 54.8 & 56.1 & 57.0 & 72.0 & 73.2 & 72.4 & 72.8 & 72.3
\\
Zlib \cite{carlini2021extracting}
& 57.2 & 61.8 & 63.0 & 64.9 & 65.9 & 87.9 & 90.0 & 90.7 & 91.4 & 91.7 & 51.5 & 53.2 & 53.7 & 54.8 & 55.1 & 78.0 & 77.4 & 77.1 & 77.3 & 77.1
\\
Min-K\% \cite{shi2023detecting}
& 62.6 & 65.8 & 66.5 & 68.4 & 69.5 & 84.2 & 87.3 & 88.1 & 89.0 & 89.6 & 53.4 & 54.6 & 55.0 & 56.4 & 56.6 & 79.7 & 79.4 & 78.9 & 79.3 & 79.1
\\
Min-K\%++ \cite{zhang2024min}
& 59.5 & 64.4 & 65.4 & 68.9 & 70.4 & 77.8 & 83.9 & 85.4 & 86.0 & 87.3 & 52.4 & 53.3 & 54.5 & 56.4 & 56.6 & 66.5 & 68.5 & 68.6 & 70.2 & 69.8
\\
NormAR
& 61.5 & 64.5 & 65.3 & 68.9 & 70.4 & 84.3 & 85.7 & 86.6 & 87.8 & 88.5 & 53.5 & 55.8 & 56.2 & 56.8 & 57.1 & 75.7 & 76.9 & 76.7 & 77.2 & 76.1
\\
AR
& 62.7 & 66.1 & 67.0 & 69.9 & 71.5 & 84.0 & 87.1 & 88.0 & 89.0 & 89.7 & 53.4 & 55.1 & 55.5 & 56.7 & 57.0 & 79.3 & 78.6 & 78.3 & 78.7 & 78.2
\\

        \vspace{-.6em} \\
    
    \toprule
    \multirow{2}{*}{}  & \multicolumn{5}{c}{\textbf{ArXiv}} & \multicolumn{5}{c}{\textbf{DM Mathematics}} & \multicolumn{5}{c}{\textbf{HackerNews}} & \multicolumn{5}{c}{\textbf{Average}}\\
    \cmidrule(lr){2-6}  \cmidrule(lr){7-11} \cmidrule(lr){12-16} \cmidrule(lr){17-21}
    \textbf{Method} 
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    \\
    \midrule

Loss \cite{yeom2018privacy} 
& 75.6 & 77.6 & 78.1 & 79.1 & 79.5 & 93.7 & 92.2 & 91.9 & 92.0 & 91.9 & 58.6 & 59.7 & 60.6 & 61.3 & 61.9 & 72.5 & 73.6 & 74.0 & 74.8 & 75.1
\\
$^\dag$Ref \cite{carlini2021extracting} 
& 61.8 & 70.8 & 71.0 & 73.2 & 74.2 & 64.1 & 47.6 & 43.8 & 43.5 & 42.9 & 52.3 & 55.0 & 57.3 & 59.8 & 62.6 & 60.4 & 63.0 & 62.1 & 63.3 & 63.6
\\
Lowercase \cite{carlini2021extracting}
& 70.3 & 72.5 & 73.7 & 74.6 & 74.8 & 86.1 & 85.3 & 92.8 & 92.8 & 90.3 & 51.0 & 52.3 & 54.0 & 54.1 & 54.8 & 67.9 & 69.6 & 71.3 & 72.2 & 72.2
\\
Zlib \cite{carlini2021extracting}
& 75.1 & 77.1 & 77.5 & 78.4 & 78.7 & 81.2 & 80.8 & 81.1 & 81.3 & 81.2 & 57.7 & 58.7 & 59.4 & 59.8 & 60.3 & 69.8 & 71.3 & 71.8 & 72.6 & 72.9
\\
Min-K\% \cite{shi2023detecting}
& 75.6 & 77.6 & 78.1 & 79.1 & 79.5 & 93.8 & 92.9 & 93.2 & 93.1 & 93.1 & 58.7 & 59.7 & 60.6 & 61.3 & 62.0 & 72.6 & 73.9 & 74.3 & 75.2 & 75.6
\\
Min-K\%++ \cite{zhang2024min}
& 60.6 & 65.8 & 67.3 & 70.0 & 71.6 & 83.0 & 75.8 & 79.1 & 77.5 & 78.3 & 55.3 & 56.8 & 58.6 & 59.9 & 61.1 & 65.0 & 66.9 & 68.4 & 69.8 & 70.7
\\
NormAR
& 77.1 & 77.7 & 78.5 & 79.0 & 79.1 & 93.6 & 94.4 & 93.9 & 94.3 & 94.9 & 59.6 & 60.0 & 60.4 & 60.7 & 61.2 & 72.2 & 73.6 & 73.9 & 75.0 & 75.3
\\
AR
& 75.6 & 77.6 & 78.1 & 79.2 & 79.6 & 94.5 & 94.2 & 94.3 & 95.1 & 95.5 & 58.6 & 59.6 & 60.6 & 61.3 & 62.2 & 72.6 & 74.0 & 74.5 & 75.7 & 76.2
\\
    
    \bottomrule
\end{tabularx}
\end{center}
% \vskip -0.1in
\end{table*}

==> tables/mimir_auroc_7_0_2_new.tex <==
\begin{table*}[b]
\caption{AUROC results on the challenging MIMIR benchmark \protect\cite{duan2024membership} with non-member sets at $\le 20\%$ 7-gram overlap threshold with a suite of Pythia models \protect\cite{biderman2024emergent}. In each column, the best result across all methods is \textbf{bolded}, with the runner-up \underline{underlined}.  Despite not requiring a reference model like the Ref method does, our methods (NormAR and AR) consistently achieve superior or comparable performance.
}
\label{tab:mimir_auroc_7_2}
\begin{center} \scriptsize
\setlength{\tabcolsep}{0.7pt}
\begin{tabularx}{\textwidth}{l *{20}{>{\centering\arraybackslash}X}@{}}
    \toprule
    \multirow{2}{*}{}  & \multicolumn{5}{c}{\textbf{Wikipedia}} & \multicolumn{5}{c}{\textbf{Github}} & \multicolumn{5}{c}{\textbf{PubMed Central}} \\
    \cmidrule(lr){2-6}  \cmidrule(lr){7-11} \cmidrule(lr){12-16}
    \textbf{Method}
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    % & 160M & 1.4B & 2.8B & 6.9B & 12B
    \\
    \midrule
    
Loss \cite{yeom2018privacy}
& 62.5 & 65.6 & 66.3 & 67.8 & 68.7 & 84.5 & 87.3 & 88.0 & 88.9 & 89.4 & 79.1 & 78.5 & 78.1 & 78.2 & 78.2
\\
% $^\dag$Ref \cite{carlini2021extracting}
% & 53.7 & 65.1 & 68.1 & 72.4 & 73.9 & 71.5 & 78.6 & 73.4 & 70.7 & 70.0 & 51.1 & 56.3 & 58.3 & 60.8 & 61.9 & 68.5 & 67.9 & 62.9 & 62.4 & 60.0
% \\
% Lowercase \cite{carlini2021extracting}
% & 61.8 & 64.4 & 64.8 & 66.9 & 67.3 & 83.4 & 86.0 & 86.9 & 88.1 & 89.1 & 50.5 & 53.5 & 54.8 & 56.1 & 57.0 & 72.0 & 73.2 & 72.4 & 72.8 & 72.3
% \\
Zlib \cite{carlini2021extracting}
& 56.5 & 61.8 & 63.0 & 64.8 & 65.1 & 88.0 & 90.0 & 90.7 & 91.3 & 91.7 & 77.4 & 77.4 & 77.1 & 77.3 & 77.3
\\
Min-K\% \cite{shi2023detecting}
& 62.5 & 65.8 & 66.6 & 68.2 & 69.2 & 84.5 & 87.3 & 88.1 & 88.9 & 89.5 & 79.6 & 79.3 & 78.9 & 79.2 & 79.4
\\
Min-K\%++ \cite{zhang2024min}
& 59.6 & 64.4 & 65.6 & 68.4 & 70.2 & 80.3 & 83.7 & 85.7 & 85.9 & 87.4 & 66.1 & 68.3 & 68.7 & 69.8 & 70.2
\\
% NormAR
% & 61.5 & 64.5 & 65.3 & 68.9 & 70.4 & 84.3 & 85.7 & 86.6 & 87.8 & 88.5 & 53.5 & 55.8 & 56.2 & 56.8 & 57.1 & 75.7 & 76.9 & 76.7 & 77.2 & 76.1
% \\
DC-PDD
& 63.2 & 66.1 & 66.9 & 68.6 & 69.1 & 89.0 & 91.1 & 91.8 & 92.2 & 92.5 & 82.0 & 80.3 & 80.2 & 80.3 & 79.9
\\
AR
& 62.9 & 66.4 & 67.2 & 69.6 & 71.0 & 88.5 & 91.0 & 91.6 & 92.2 & 92.5 & 82.4 & 81.0 & 80.8 & 80.7 & 80.7
\\

        \vspace{-.6em} \\
    
    \toprule
    \multirow{2}{*}{}  & \multicolumn{5}{c}{\textbf{ArXiv}} & \multicolumn{5}{c}{\textbf{DM Mathematics}} & \multicolumn{5}{c}{\textbf{Average}}\\
    \cmidrule(lr){2-6}  \cmidrule(lr){7-11} \cmidrule(lr){12-16}
    \textbf{Method} 
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    % & 160M & 1.4B & 2.8B & 6.9B & 12B
    \\
    \midrule

Loss \cite{yeom2018privacy} 
& 75.3 & 77.6 & 78.0 & 79.0 & 79.5 & 93.9 & 92.2 & 91.9 & 92.0 & 91.9 & 79.1 & 80.2 & 80.5 & 81.2 & 81.5
\\
% $^\dag$Ref \cite{carlini2021extracting} 
% & 61.8 & 70.8 & 71.0 & 73.2 & 74.2 & 64.1 & 47.6 & 43.8 & 43.5 & 42.9 & 52.3 & 55.0 & 57.3 & 59.8 & 62.6 & 60.4 & 63.0 & 62.1 & 63.3 & 63.6
% \\
% Lowercase \cite{carlini2021extracting}
% & 70.3 & 72.5 & 73.7 & 74.6 & 74.8 & 86.1 & 85.3 & 92.8 & 92.8 & 90.3 & 51.0 & 52.3 & 54.0 & 54.1 & 54.8 & 67.9 & 69.6 & 71.3 & 72.2 & 72.2
% \\
Zlib \cite{carlini2021extracting}
& 74.4 & 77.1 & 77.5 & 78.3 & 78.6 & 80.3 & 80.7 & 81.0 & 81.1 & 81.0 & 75.3 & 77.4 & 77.9 & 78.6 & 78.7
\\
Min-K\% \cite{shi2023detecting}
& 75.3 & 77.6 & 78.0 & 79.0 & 79.5 & 94.0 & 92.8 & 93.1 & 93.0 & 93.2 & 79.2 & 80.6 & 80.9 & 81.7 & 82.2
\\
Min-K\%++ \cite{zhang2024min}
& 61.6 & 65.5 & 67.7 & 69.5 & 71.4 & 79.1 & 74.9 & 78.5 & 76.5 & 77.7 & 69.3 & 71.4 & 73.2 & 74.0 & 75.4
\\
% NormAR
% & 77.1 & 77.7 & 78.5 & 79.0 & 79.1 & 93.6 & 94.4 & 93.9 & 94.3 & 94.9 & 59.6 & 60.0 & 60.4 & 60.7 & 61.2 & 72.2 & 73.6 & 73.9 & 75.0 & 75.3
% \\
DC-PDD
& 75.5 & 77.8 & 78.1 & 79.0 & 79.5 & 91.4 & 91.3 & 91.6 & 91.3 & 91.4 & \textbf{80.2} & 81.3 & 81.7 & 82.3 & 82.5
\\
AR
& 74.2 & 77.3 & 77.9 & 79.2 & 80.0 & 91.1 & 93.0 & 94.0 & 93.5 & 93.5 & 79.8 & \textbf{81.7} & \textbf{82.3} & \textbf{83.0} & \textbf{83.5}
\\
    
    \bottomrule
\end{tabularx}
\end{center}
% \vskip -0.1in
\end{table*}

==> tables/mimir_tpr.tex <==
\begin{table*}[b]
\caption{TPR at low FPR (FPR=5\%) results on the challenging MIMIR benchmark \cite{mimir} with a suite of Pythia models \cite{pythia}. In each column, the best result across all methods is \textbf{bolded}, with the runner-up \underline{underlined}. 
$^\dag$Ref relies on a reference LLM.
$^\ddag$Neighbor induces significant extra computational cost than others ($25\times$ in this case), for which reason we don't run on the 12B model. Despite not requiring a reference model like the Ref method does, our methods consistently achieve superior or comparable performance.\\
13-0.8
}
\label{tab:mimir_auroc}
\begin{center} \scriptsize
\setlength{\tabcolsep}{0.7pt}
\begin{tabularx}{\textwidth}{l *{20}{>{\centering\arraybackslash}X}@{}}
    \toprule
    \multirow{2}{*}{}  & \multicolumn{5}{c}{\textbf{Wikipedia}} & \multicolumn{5}{c}{\textbf{Github}} & \multicolumn{5}{c}{\textbf{Pile CC}} & \multicolumn{5}{c}{\textbf{PubMed Central}} \\
    \cmidrule(lr){2-6}  \cmidrule(lr){7-11} \cmidrule(lr){12-16} \cmidrule(lr){17-21}
    \textbf{Method}
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    \\
    \midrule
    
Loss \cite{yeom2018privacy} 
& 4.2 & 4.7 & 4.7 & 5.1 & 5.0 & 22.6 & 32.1 & 33.6 & 38.5 & 40.7 & 3.1 & 5.0 & 4.8 & 4.9 & 5.4 & 4.0 & 4.4 & 4.3 & 4.9 & 5.1
\\
$^\dag$Ref \cite{carlini2021extracting} 
& 6.1 & 5.3 & 5.5 & 5.6 & 5.5 & 23.4 & 14.8 & 14.9 & 15.4 & 16.5 & 5.5 & 5.6 & 5.8 & 5.8 & 7.4 & 5.7 & 4.1 & 4.0 & 5.9 & 7.3
\\
Lowercase \cite{carlini2021extracting}
& 4.6 & 4.5 & 4.9 & 5.2 & 5.5 & 24.4 & 32.2 & 34.3 & 38.1 & 38.0 & 3.4 & 5.3 & 5.3 & 6.2 & 6.3 & 3.5 & 5.0 & 5.3 & 6.0 & 4.9
\\
Zlib \cite{carlini2021extracting}
& 4.2 & 5.7 & 5.9 & 6.3 & 6.6 & 25.0 & 32.8 & 36.1 & 40.1 & 40.8 & 4.0 & 5.1 & 5.4 & 6.2 & 6.6 & 3.8 & 3.6 & 3.5 & 4.3 & 4.4
\\
$^\ddag$Neighbor \cite{mia_neighbor} 
& 4.0 & 4.5 & 4.9 & 5.8 & / & 24.7 & 31.6 & 29.8 & 34.1 & / & 3.9 & 3.6 & 4.0 & 5.3 & / & 3.9 & 3.7 & 4.5 & 4.5 & /
\\
Min-K\% \cite{shi2023detecting}
& 4.2 & 4.7 & 5.2 & 6.5 & 8.1 & 22.6 & 31.9 & 34.0 & 39.0 & 39.5 & 4.2 & 4.4 & 3.9 & 4.4 & 4.9 & 4.7 & 4.6 & 4.5 & 5.1 & 5.4
\\
Min-K\%++ \cite{zhang2024min}
& 5.3 & 5.8 & 8.5 & 11.4 & 10.2 & 25.0 & 33.0 & 34.2 & 38.2 & 40.0 & 4.7 & 5.0 & 4.8 & 6.0 & 5.7 & 3.9 & 6.3 & 6.5 & 7.4 & 8.4
\\
Normalized Temp
& 4.3 & 5.8 & 8.5 & 11.4 & 10.2 & 25.5 & 31.6 & 33.1 & 36.1 & 38.4 & 6.2 & 4.7 & 4.3 & 6.0 & 5.1 & 4.9 & 5.8 & 6.0 & 6.9 & 8.4
\\
Temp - Original
& 5.3 & 6.1 & 8.0 & 10.3 & 11.0 & 24.2 & 32.4 & 34.4 & 37.4 & 42.2 & 5.8 & 4.9 & 6.4 & 7.1 & 7.0 & 5.6 & 5.4 & 4.9 & 6.0 & 6.2
\\

        \vspace{-.6em} \\
    
    \toprule
    \multirow{2}{*}{}  & \multicolumn{5}{c}{\textbf{ArXiv}} & \multicolumn{5}{c}{\textbf{DM Mathematics}} & \multicolumn{5}{c}{\textbf{HackerNews}} & \multicolumn{5}{c}{\textbf{Average}}\\
    \cmidrule(lr){2-6}  \cmidrule(lr){7-11} \cmidrule(lr){12-16} \cmidrule(lr){17-21}
    \textbf{Method} 
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    \\
    \midrule

Loss \cite{yeom2018privacy} 
& 4.0 & 4.8 & 4.6 & 5.4 & 5.9 & 3.8 & 4.3 & 4.1 & 4.1 & 4.2 & 5.0 & 4.8 & 5.5 & 5.9 & 6.4 & 6.7 & 8.6 & 8.8 & 9.8 & 10.4
\\
$^\dag$Ref \cite{carlini2021extracting} 
& 5.2 & 5.4 & 5.9 & 6.8 & 7.7 & 5.3 & 3.6 & 4.9 & 5.4 & 5.8 & 5.2 & 6.3 & 7.6 & 7.0 & 7.7 & 8.1 & 6.4 & 6.9 & 7.4 & 8.3
\\
Lowercase \cite{carlini2021extracting}
& 5.1 & 4.7 & 5.4 & 5.6 & 5.0 & 5.6 & 6.2 & 5.5 & 6.8 & 5.5 & 5.2 & 5.2 & 6.3 & 6.6 & 6.7 & 7.4 & 9.0 & 9.6 & 10.6 & 10.3
\\
Zlib \cite{carlini2021extracting}
& 2.9 & 4.3 & 4.1 & 4.6 & 4.3 & 4.1 & 5.0 & 4.6 & 4.3 & 4.3 & 5.0 & 5.5 & 5.8 & 5.6 & 5.7 & 7.0 & 8.9 & 9.3 & 10.2 & 10.4
\\
$^\ddag$Neighbor \cite{mia_neighbor} 
& 4.7 & 4.8 & 4.4 & 4.1 & / & 5.6 & 4.4 & 4.5 & 4.5 & / & 6.5 & 5.2 & 5.3 & 5.7 & / & 7.6 & 8.3 & 8.2 & 9.1 & /
\\
Min-K\% \cite{shi2023detecting}
& 4.0 & 3.9 & 4.2 & 4.6 & 4.8 & 4.5 & 4.1 & 4.5 & 4.5 & 4.6 & 4.9 & 5.1 & 5.9 & 6.3 & 6.2 & 7.0 & 8.4 & 8.9 & 10.1 & 10.5
\\
Min-K\%++ \cite{zhang2024min}
& 4.3 & 6.0 & 6.7 & 7.4 & 7.7 & 5.1 & 5.4 & 5.3 & 6.2 & 5.6 & 4.4 & 3.7 & 4.9 & 6.4 & 4.7 & 7.5 & 9.3 & 10.1 & 11.9 & 11.8
\\
Normalized Temp
& 3.6 & 6.2 & 5.4 & 3.8 & 7.7 & 4.2 & 6.3 & 6.1 & 6.5 & 5.4 & 6.7 & 4.2 & 5.6 & 4.4 & 4.7 & 7.9 & 9.2 & 9.9 & 10.7 & 11.4
\\
Temp - Original
& 5.3 & 4.1 & 3.7 & 4.4 & 6.2 & 5.6 & 4.9 & 4.0 & 5.6 & 4.5 & 6.1 & 5.0 & 6.2 & 5.8 & 7.2 & 8.3 & 9.0 & 9.7 & 10.9 & 12.0
\\
    
    \bottomrule
\end{tabularx}
\end{center}
% \vskip -0.1in
\end{table*}

==> tables/mimir_tpr_13_0.2.tex <==
\begin{table*}[b]
\caption{TPR at low FPR (FPR=5\%) results on the challenging MIMIR benchmark \cite{mimir} with a suite of Pythia models \cite{pythia}. In each column, the best result across all methods is \textbf{bolded}, with the runner-up \underline{underlined}. 
$^\dag$Ref relies on a reference LLM.
Despite not requiring a reference model like the Ref method does, our methods consistently achieve superior or comparable performance.\\
13-0.2
}
\label{tab:mimir_auroc}
\begin{center} \scriptsize
\setlength{\tabcolsep}{0.7pt}
\begin{tabularx}{\textwidth}{l *{20}{>{\centering\arraybackslash}X}@{}}
    \toprule
    \multirow{2}{*}{}  & \multicolumn{5}{c}{\textbf{Wikipedia}} & \multicolumn{5}{c}{\textbf{Github}} & \multicolumn{5}{c}{\textbf{Pile CC}} & \multicolumn{5}{c}{\textbf{PubMed Central}} \\
    \cmidrule(lr){2-6}  \cmidrule(lr){7-11} \cmidrule(lr){12-16} \cmidrule(lr){17-21}
    \textbf{Method}
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    \\
    \midrule
    
Loss \cite{yeom2018privacy} 
& 7.9 & 10.1 & 11.5 & 12.1 & 12.6 & 36.9 & 45.1 & 49.7 & 54.1 & 53.8 & 3.6 & 7.3 & 7.5 & 8.2 & 8.9 & 4.7 & 4.8 & 5.6 & 5.9 & 5.7
\\
$^\dag$Ref \cite{carlini2021extracting} 
& 6.0 & 9.5 & 10.8 & 12.7 & 12.3 & 33.6 & 23.4 & 19.2 & 19.3 & 20.0 & 5.8 & 8.9 & 10.3 & 12.9 & 13.4 & 4.8 & 4.9 & 5.0 & 7.4 & 9.2
\\
Lowercase \cite{carlini2021extracting}
& 6.5 & 9.9 & 9.7 & 10.8 & 10.6 & 52.4 & 56.2 & 57.3 & 59.5 & 61.4 & 5.2 & 8.5 & 8.2 & 9.6 & 10.6 & 5.2 & 6.5 & 7.1 & 6.8 & 8.9
\\
Zlib \cite{carlini2021extracting}
& 7.0 & 8.6 & 9.6 & 10.2 & 10.7 & 52.8 & 57.8 & 59.9 & 62.3 & 62.7 & 5.5 & 7.4 & 7.9 & 9.1 & 9.9 & 4.1 & 4.6 & 5.1 & 5.0 & 5.7
\\
Min-K\% \cite{shi2023detecting}
& 7.9 & 9.3 & 11.5 & 12.1 & 12.0 & 36.9 & 45.1 & 49.9 & 54.1 & 53.8 & 4.6 & 6.2 & 5.5 & 6.2 & 6.6 & 4.3 & 5.9 & 5.7 & 6.1 & 6.7
\\
Min-K\%++ \cite{zhang2024min}
& 6.9 & 10.2 & 11.1 & 13.7 & 14.7 & 33.8 & 44.5 & 45.3 & 50.0 & 52.4 & 4.2 & 7.7 & 7.3 & 7.9 & 9.4 & 3.8 & 6.4 & 6.4 & 6.2 & 8.5
\\
Normalized Temp
& 7.2 & 10.1 & 9.5 & 12.2 & 12.6 & 38.6 & 43.0 & 45.9 & 49.7 & 53.2 & 4.2 & 7.7 & 6.2 & 7.8 & 8.1 & 4.8 & 6.4 & 5.1 & 7.2 & 7.6
\\
Temp - Original
& 7.1 & 10.2 & 10.3 & 13.1 & 14.0 & 34.2 & 45.5 & 49.1 & 52.3 & 52.7 & 3.6 & 6.1 & 6.6 & 8.0 & 7.5 & 4.5 & 6.2 & 6.9 & 7.1 & 8.2
\\

        \vspace{-.6em} \\
    
    \toprule
    \multirow{2}{*}{}  & \multicolumn{5}{c}{\textbf{ArXiv}} & \multicolumn{5}{c}{\textbf{DM Mathematics}} & \multicolumn{5}{c}{\textbf{HackerNews}} & \multicolumn{5}{c}{\textbf{Average}}\\
    \cmidrule(lr){2-6}  \cmidrule(lr){7-11} \cmidrule(lr){12-16} \cmidrule(lr){17-21}
    \textbf{Method} 
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    \\
    \midrule

Loss \cite{yeom2018privacy} 
& 6.8 & 7.7 & 8.1 & 8.9 & 9.8 & 19.2 & 14.8 & 12.2 & 11.8 & 12.1 & 5.7 & 5.0 & 6.3 & 6.3 & 7.2 & 10.6 & 9.2 & 8.9 & 9.0 & 9.7
\\
$^\dag$Ref \cite{carlini2021extracting} 
& 5.7 & 7.9 & 8.4 & 9.9 & 9.8 & 5.8 & 2.1 & 3.0 & 2.8 & 2.6 & 5.5 & 6.1 & 7.7 & 7.1 & 9.3 & 5.7 & 5.4 & 6.4 & 6.6 & 7.2
\\
Lowercase \cite{carlini2021extracting}
& 7.9 & 7.7 & 7.5 & 9.5 & 9.3 & 10.4 & 9.5 & 9.4 & 15.3 & 10.8 & 5.0 & 5.1 & 6.5 & 6.8 & 6.8 & 7.8 & 7.4 & 7.8 & 10.5 & 9.0
\\
Zlib \cite{carlini2021extracting}
& 6.4 & 7.6 & 8.8 & 10.7 & 11.1 & 16.0 & 11.3 & 10.0 & 10.9 & 10.7 & 6.6 & 5.9 & 6.4 & 6.7 & 7.1 & 9.7 & 8.3 & 8.4 & 9.4 & 9.6
\\
Min-K\% \cite{shi2023detecting}
& 7.0 & 7.8 & 8.4 & 9.3 & 10.7 & 19.2 & 14.8 & 12.2 & 12.1 & 12.2 & 5.4 & 6.4 & 6.8 & 6.3 & 7.9 & 10.5 & 9.7 & 9.1 & 9.2 & 10.3
\\
Min-K\%++ \cite{zhang2024min}
& 6.8 & 7.2 & 8.3 & 11.0 & 10.9 & 9.0 & 10.6 & 11.3 & 11.2 & 11.6 & 4.3 & 4.0 & 4.5 & 6.6 & 5.2 & 6.7 & 7.3 & 8.0 & 9.6 & 9.2
\\
Normalized Temp
& 6.0 & 7.1 & 7.9 & 10.3 & 10.4 & 19.2 & 16.3 & 15.7 & 19.7 & 16.7 & 4.2 & 6.6 & 5.5 & 7.1 & 5.5 & 9.8 & 10.0 & 9.7 & 12.4 & 10.9
\\
Temp - Original
& 6.9 & 8.1 & 8.7 & 10.4 & 9.9 & 21.6 & 21.0 & 19.9 & 21.4 & 20.6 & 5.9 & 5.4 & 8.1 & 7.2 & 6.1 & 11.5 & 11.5 & 12.2 & 13.0 & 12.2
\\
    
    \bottomrule
\end{tabularx}
\end{center}
% \vskip -0.1in
\end{table*}

==> tables/mimir_tpr_7_0.2.tex <==
\begin{table*}[b]
\caption{TPR at low FPR (FPR=5\%) results on the challenging MIMIR benchmark \cite{mimir} with a suite of Pythia models \cite{pythia}. In each column, the best result across all methods is \textbf{bolded}, with the runner-up \underline{underlined}. 
$^\dag$Ref relies on a reference LLM.
Despite not requiring a reference model like the Ref method does, our methods consistently achieve superior or comparable performance.\\
7-0.2
}
\label{tab:mimir_auroc}
\begin{center} \scriptsize
\setlength{\tabcolsep}{0.7pt}
\begin{tabularx}{\textwidth}{l *{20}{>{\centering\arraybackslash}X}@{}}
    \toprule
    \multirow{2}{*}{}  & \multicolumn{5}{c}{\textbf{Wikipedia}} & \multicolumn{5}{c}{\textbf{Github}} & \multicolumn{5}{c}{\textbf{Pile CC}} & \multicolumn{5}{c}{\textbf{PubMed Central}} \\
    \cmidrule(lr){2-6}  \cmidrule(lr){7-11} \cmidrule(lr){12-16} \cmidrule(lr){17-21}
    \textbf{Method}
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    \\
    \midrule
    
Loss \cite{yeom2018privacy} 
& 19.6 & 23.7 & 22.8 & 24.0 & 24.4 & 41.4 & 58.2 & 57.1 & 61.9 & 61.2 & 8.3 & 11.1 & 11.4 & 13.7 & 13.9 & 29.9 & 31.0 & 32.0 & 30.5 & 32.6
\\
$^\dag$Ref \cite{carlini2021extracting} 
& 8.7 & 21.3 & 19.5 & 20.9 & 20.4 & 26.5 & 27.2 & 23.9 & 22.4 & 20.5 & 6.9 & 12.7 & 14.4 & 17.1 & 17.9 & 20.6 & 6.5 & 5.1 & 4.1 & 4.3
\\
Lowercase \cite{carlini2021extracting}
& 20.7 & 21.4 & 21.5 & 22.8 & 23.9 & 63.4 & 67.5 & 67.5 & 66.0 & 67.9 & 8.4 & 10.1 & 9.5 & 12.0 & 11.0 & 21.4 & 25.3 & 18.9 & 20.0 & 17.1
\\
Zlib \cite{carlini2021extracting}
& 14.4 & 20.2 & 19.5 & 20.5 & 21.5 & 63.8 & 70.5 & 71.3 & 74.3 & 75.7 & 9.5 & 12.7 & 12.4 & 13.9 & 14.2 & 26.7 & 29.5 & 29.3 & 29.1 & 28.1
\\
Min-K\% \cite{shi2023detecting}
& 19.9 & 22.7 & 23.0 & 23.7 & 26.1 & 41.4 & 58.2 & 56.0 & 61.9 & 60.4 & 8.4 & 11.8 & 12.2 & 14.5 & 14.8 & 35.2 & 35.6 & 35.0 & 34.2 & 34.0
\\
Min-K\%++ \cite{zhang2024min}
& 15.7 & 19.7 & 22.4 & 23.4 & 26.0 & 36.9 & 54.1 & 54.9 & 56.0 & 58.2 & 7.0 & 10.3 & 10.9 & 12.8 & 11.4 & 20.0 & 20.4 & 21.4 & 24.8 & 22.8
\\
Normalized Temp
& 16.6 & 21.2 & 22.5 & 24.4 & 26.5 & 47.8 & 51.9 & 53.7 & 59.0 & 64.2 & 8.1 & 10.6 & 10.6 & 11.8 & 12.0 & 16.5 & 17.3 & 26.7 & 29.7 & 21.4
\\
Temp - Original
& 20.5 & 25.1 & 25.2 & 24.9 & 28.5 & 40.3 & 54.9 & 54.1 & 57.5 & 62.7 & 9.9 & 10.9 & 12.5 & 13.6 & 12.9 & 31.0 & 33.6 & 33.8 & 34.6 & 34.6
\\

        \vspace{-.6em} \\
    
    \toprule
    \multirow{2}{*}{}  & \multicolumn{5}{c}{\textbf{ArXiv}} & \multicolumn{5}{c}{\textbf{DM Mathematics}} & \multicolumn{5}{c}{\textbf{HackerNews}} & \multicolumn{5}{c}{\textbf{Average}}\\
    \cmidrule(lr){2-6}  \cmidrule(lr){7-11} \cmidrule(lr){12-16} \cmidrule(lr){17-21}
    \textbf{Method} 
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    & 160M & 1.4B & 2.8B & 6.9B & 12B
    \\
    \midrule

Loss \cite{yeom2018privacy} 
& 29.0 & 32.0 & 34.2 & 37.0 & 36.2 & 79.8 & 62.9 & 59.6 & 62.9 & 62.9 & 8.7 & 11.0 & 11.6 & 12.2 & 14.1 & 31.0 & 32.8 & 32.7 & 34.6 & 35.0
\\
$^\dag$Ref \cite{carlini2021extracting} 
& 10.4 & 20.4 & 19.0 & 21.8 & 22.6 & 4.5 & 4.5 & 6.7 & 5.6 & 3.4 & 5.9 & 7.4 & 8.4 & 9.8 & 11.1 & 11.9 & 14.3 & 13.9 & 14.5 & 14.3
\\
Lowercase \cite{carlini2021extracting}
& 25.2 & 26.6 & 25.0 & 27.6 & 28.2 & 58.4 & 65.2 & 66.3 & 67.4 & 64.0 & 6.8 & 5.9 & 7.4 & 8.0 & 7.4 & 29.2 & 31.7 & 30.9 & 32.0 & 31.4
\\
Zlib \cite{carlini2021extracting}
& 28.0 & 30.6 & 34.6 & 33.6 & 33.4 & 22.5 & 16.9 & 16.9 & 16.9 & 16.9 & 11.3 & 10.7 & 10.5 & 11.8 & 12.7 & 25.2 & 27.3 & 27.8 & 28.6 & 28.9
\\
Min-K\% \cite{shi2023detecting}
& 29.0 & 32.2 & 34.2 & 37.0 & 36.4 & 79.8 & 69.7 & 69.7 & 69.7 & 69.7 & 8.8 & 11.0 & 11.6 & 12.4 & 13.9 & 31.8 & 34.5 & 34.5 & 36.2 & 36.5
\\
Min-K\%++ \cite{zhang2024min}
& 12.0 & 12.8 & 16.8 & 17.0 & 22.6 & 53.9 & 36.0 & 31.5 & 34.8 & 29.2 & 7.7 & 8.5 & 8.8 & 9.3 & 9.0 & 21.9 & 23.1 & 23.8 & 25.4 & 25.6
\\
Normalized Temp
& 30.4 & 29.6 & 32.8 & 34.2 & 35.0 & 84.3 & 87.6 & 70.8 & 76.4 & 82.0 & 10.1 & 9.6 & 11.9 & 12.5 & 11.3 & 30.5 & 32.5 & 32.7 & 35.4 & 36.1
\\
Temp - Original
& 29.4 & 32.2 & 34.2 & 40.2 & 36.2 & 85.4 & 75.3 & 83.1 & 84.3 & 85.4 & 9.8 & 11.0 & 11.9 & 13.2 & 14.2 & 32.3 & 34.7 & 36.4 & 38.3 & 39.2
\\
    
    \bottomrule
\end{tabularx}
\end{center}
% \vskip -0.1in
\end{table*}

==> tables/online_detection.tex <==
\begin{table}[ht]
\caption{AUROC results in the online detection setting with Pythia models.}
\vspace{-20pt}
\label{tab:online}
\begin{tabular}{lccc}\\\toprule  
& 2.8B & 6.9B & 12B \\\midrule
Loss \cite{yeom2018privacy} & 56.6 & 57.2 & 56.6 \\ 
Zlib \cite{carlini2021extracting} & 55.9 & 56.6 & 56.0 \\ 
Min-K\%\cite{shi2023detecting} & \textbf{58.4} & \textbf{58.8} & 58.4 \\ 
Min-K\%++\cite{zhang2024min} & 56.4 & 57.9 & 57.5 \\
NormAR & 57.5 & 58.4 & 58.3 \\
AR & 57.9 & \textbf{58.8} & \textbf{59.3} \\
\bottomrule
\end{tabular}
\end{table}

==> tables/wiki_main_results.tex <==
\begin{table*}[t]
\centering
%\footnotesize
\caption{AUROC results on WikiMIA benchmark \cite{shi2023detecting}. \textit{Ori.} and \textit{Para.} denote the original and paraphrased settings, respectively. \textbf{Bolded} number shows the best result within each column across all methods.}
\label{tab:wikimia_main}
\resizebox{0.98\textwidth}{!}{%
\begin{tabular}{llcccccccccccc}\\
\toprule
& & \multicolumn{2}{c}{\textbf{Pythia-2.8B}} & \multicolumn{2}{c}{\textbf{Pythia-6.9B}} & \multicolumn{2}{c}{\textbf{Pythia-12B}} & \multicolumn{2}{c}
{\textbf{OPT-13B}} & \multicolumn{2}{c}{\textbf{NeoX-20B}} & \multicolumn{2}{c}{\textbf{Average}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14}  
\textbf{Len.} & \textbf{Method} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} \\
\midrule
    
\multirow{8}{*}{32}
 & Loss \cite{yeom2018privacy} 
 & 61.4 & 61.6 & 63.8 & 64.1 & 65.5 & 65.6 & 62.6 & 62.4 & 68.8 & 68.3 & 64.4 & 64.4
 \\
 & Ref \cite{carlini2021extracting} 
 & 61.3 & 61.2 & 63.6 & 63.5 & 65.1 & 64.8 & 65.9 & 65.5 & 67.3 & 66.2 & 64.6 & 64.2
 \\ 
 & Lowercase \cite{carlini2021extracting} 
 & 60.9 & 60.3 & 62.2 & 61.7 & 65.2 & 64.7 & 61.9 & 60.5 & 68.2 & 66.3 & 63.7 & 62.7
 \\ 
 & Zlib \cite{carlini2021extracting} 
 & 62.1 & 62.3 & 64.4 & 64.2 & 65.9 & 65.9 & 63.3 & 63.0 & 69.1 & 68.3 & 65.0 & 64.7
 \\ 
 & Min-K\% \cite{shi2023detecting} 
 & 61.8 & 61.7 & 66.3 & 65.2 & 68.2 & 67.1 & 64.0 & 63.2 & 71.6 & 69.7 & 66.4 & 65.4
 \\ 
 & Min-K\%++ \cite{zhang2024min}
 & 64.4 & 62.4 & 70.3 & 68.0 & 73.2 & 70.6 & 66.8 & 64.4 & 75.2 & 70.1 & 70.0 & 67.1
 \\ 
 & Normalized Temp
 & 65.0 & 63.4 & 70.6 & 68.5 & 73.3 & 71.1 & 65.8 & 63.6 & 75.8 & 70.9 & 70.1 & 67.5
 \\
 & Temp - Original
 & 64.6 & 63.8 & 70.5 & 69.1 & 72.7 & 71.1 & 65.5 & 64.0 & 76.4 & 73.3 & 69.9 & 68.3
 \\
\midrule

\multirow{8}{*}{64}
 & Loss \cite{yeom2018privacy} 
 & 58.4 & 56.5 & 60.7 & 59.3 & 61.8 & 59.9 & 58.7 & 57.1 & 66.4 & 63.8 & 61.2 & 59.3
 \\ 
 & Ref \cite{carlini2021extracting} 
 & 59.6 & 59.2 & 62.4 & 62.9 & 63.0 & 63.0 & 63.3 & 63.9 & 65.8 & 65.6 & 62.8 & 62.9
 \\ 
 & Lowercase \cite{carlini2021extracting} 
 & 57.8 & 56.1 & 58.2 & 57.7 & 59.5 & 59.0 & 58.6 & 57.2 & 65.6 & 64.0 & 59.9 & 58.8
 \\ 
 & Zlib \cite{carlini2021extracting} 
 & 60.6 & 59.0 & 62.6 & 61.6 & 63.4 & 61.9 & 60.7 & 59.3 & 67.7 & 65.9 & 63.0 & 61.5
 \\  
 & Min-K\% \cite{shi2023detecting} 
 & 61.2 & 56.8 & 65.0 & 61.1 & 67.4 & 62.3 & 62.2 & 58.0 & 72.0 & 65.8 & 65.6 & 60.8
 \\ 
 & Min-K\%++ \cite{zhang2024min}
 & 65.0 & 58.5 & 71.6 & 64.8 & 72.4 & 65.5 & 67.4 & 59.9 & 76.1 & 66.7 & 70.5 & 63.1
 \\  
 & Normalized Temp
 & 64.3 & 59.0 & 70.7 & 65.3 & 70.8 & 65.4 & 65.5 & 59.7 & 76.3 & 67.6 & 69.5 & 63.4
 \\
 & Temp - Original
 & 62.1 & 58.3 & 68.6 & 64.4 & 69.2 & 65.2 & 63.7 & 59.4 & 75.7 & 68.8 & 67.9 & 63.2
 \\
\midrule

\multirow{8}{*}{128} 
 & Loss \cite{yeom2018privacy} 
 & 62.8 & 62.3 & 65.1 & 64.7 & 65.6 & 65.4 & 63.2 & 62.4 & 70.2 & 69.3 & 65.4 & 64.8
 \\ 
 & Ref \cite{carlini2021extracting} 
 & 59.6 & 59.5 & 63.3 & 62.9 & 63.5 & 63.9 & 64.7 & 65.0 & 67.8 & 67.7 & 63.8 & 63.8
 \\ 
 & Lowercase \cite{carlini2021extracting} 
 & 59.5 & 59.6 & 60.5 & 60.0 & 60.6 & 60.4 & 59.5 & 58.6 & 66.8 & 66.7 & 61.4 & 61.1
 \\ 
 & Zlib \cite{carlini2021extracting} 
 & 65.0 & 65.0 & 67.6 & 67.4 & 67.7 & 68.1 & 65.1 & 65.1 & 71.9 & 71.7 & 67.5 & 67.5
 \\ 
 & Min-K\% \cite{shi2023detecting} 
 & 66.9 & 64.7 & 69.5 & 67.0 & 69.9 & 68.6 & 68.2 & 65.6 & 75.3 & 72.4 & 70.0 & 67.7
 \\ 
 & Min-K\%++ \cite{zhang2024min}
 & 66.8 & 63.4 & 70.7 & 66.8 & 71.8 & 68.9 & 70.7 & 65.5 & 76.3 & 71.6 & 71.3 & 67.2
 \\  
 & Normalized Temp
 & 67.7 & 65.3 & 71.7 & 68.6 & 72.1 & 70.3 & 72.1 & 67.8 & 76.3 & 72.4 & 72.0 & 68.9
 \\
 & Temp - Original
 & 67.4 & 65.0 & 71.7 & 68.6 & 72.4 & 69.9 & 69.6 & 66.0 & 77.8 & 73.6 & 71.8 & 68.6
 \\
\midrule

\multirow{8}{*}{256} 
 & Loss \cite{yeom2018privacy} 
 & 67.8 & - & 68.6 & - & 68.3 & - & 65.1 & - & 70.9 & - & 68.1 & -
 \\ 
 & Ref \cite{carlini2021extracting} 
 & 63.6 & - & 64.1 & - & 64.6 & - & 71.2 & - & 69.3 & - & 66.6 & -
 \\ 
 & Lowercase \cite{carlini2021extracting} 
 & 62.9 & - & 59.5 & - & 62.1 & - & 63.0 & - & 66.5 & - & 62.8 & -
 \\ 
 & Zlib \cite{carlini2021extracting} 
 & 69.3 & - & 69.8 & - & 70.8 & - & 67.4 & - & 72.8 & - & 70.0 & -
 \\ 
 & Min-K\% \cite{shi2023detecting} 
 & 70.0 & - & 71.7 & - & 73.3 & - & 68.2 & - & 76.7 & - & 72.0 & -
 \\ 
 & Min-K\%++ \cite{zhang2024min}
 & 63.9 & - & 65.5 & - & 66.1 & - & 68.1 & - & 69.4 & - & 66.6 & -
 \\  
 & Normalized Temp
 & 66.0 & - & 68.5 & - & 67.2 & - & 71.2 & - & 72.6 & - & 69.1 & -
 \\
 & Temp - Original
 & 70.1 & - & 72.6 & - & 72.3 & - & 70.9 & - & 77.2 & - & 72.6 & -
 \\
\bottomrule


\end{tabular}
}

\end{table*}

==> tables/wiki_tpr_results.tex <==
\begin{table*}[t]
\centering
%\footnotesize
\caption{TPR at low FPR (FPR=5\%) results on WikiMIA benchmark \cite{shi2023detecting}. \textit{Ori.} and \textit{Para.} denote the original and paraphrased settings, respectively. \textbf{Bolded} number shows the best result within each column across all methods.}
\label{tab:wikimia_main}
\resizebox{0.98\textwidth}{!}{%
\begin{tabular}{llcccccccccccc}\\
\toprule
& & \multicolumn{2}{c}{\textbf{Pythia-2.8B}} & \multicolumn{2}{c}{\textbf{Pythia-6.9B}} & \multicolumn{2}{c}{\textbf{Pythia-12B}} & \multicolumn{2}{c}
{\textbf{OPT-13B}} & \multicolumn{2}{c}{\textbf{NeoX-20B}} & \multicolumn{2}{c}{\textbf{Average}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14}  
\textbf{Len.} & \textbf{Method} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} \\
\midrule


\multirow{8}{*}{32}
 & Loss \cite{yeom2018privacy} 
 & 14.7 & 14.2 & 14.2 & 15.0 & 18.1 & 16.3 & 11.9 & 14.5 & 19.6 & 18.9 & 15.7 & 15.8
 \\
 & Ref \cite{carlini2021extracting} 
 & 6.2 & 7.2 & 6.7 & 6.2 & 9.8 & 8.8 & 9.3 & 8.3 & 16.3 & 14.2 & 9.7 & 8.9
 \\ 
 & Lowercase \cite{carlini2021extracting} 
 & 11.1 & 11.6 & 10.6 & 11.9 & 14.7 & 15.5 & 9.3 & 7.5 & 16.5 & 14.7 & 12.4 & 12.2
 \\ 
 & Zlib \cite{carlini2021extracting} 
 & 15.8 & 14.5 & 16.3 & 12.7 & 17.6 & 15.0 & 13.7 & 13.4 & 19.4 & 17.3 & 16.6 & 14.6
 \\ 
 & Min-K\% \cite{shi2023detecting} 
 & 17.1 & 16.5 & 17.8 & 21.7 & 20.9 & 19.6 & 17.8 & 14.2 & 28.4 & 18.3 & 20.4 & 18.1
 \\ 
 & Min-K\%++ \cite{zhang2024min}
 & 12.4 & 14.0 & 14.5 & 16.3 & 18.6 & 16.5 & 11.1 & 10.3 & 22.2 & 15.2 & 15.8 & 14.5
 \\ 
 & Normalized Temp
 & 17.6 & 11.9 & 18.1 & 15.0 & 21.7 & 17.3 & 8.0 & 12.4 & 24.5 & 19.1 & 18.0 & 15.1
 \\
 & Temp - Original
 & 16.8 & 14.2 & 21.2 & 17.8 & 24.0 & 24.3 & 15.0 & 15.8 & 26.4 & 23.8 & 20.7 & 19.2
 \\
\midrule

\multirow{9}{*}{64}
 & Loss \cite{yeom2018privacy} 
 & 10.2 & 9.5 & 13.4 & 10.6 & 8.1 & 11.3 & 10.6 & 11.6 & 12.7 & 15.8 & 11.0 & 11.8
 \\ 
 & Ref \cite{carlini2021extracting} 
 & 10.6 & 13.0 & 12.0 & 16.2 & 11.6 & 15.5 & 8.8 & 9.5 & 14.4 & 15.5 & 11.5 & 13.9
 \\ 
 & Lowercase \cite{carlini2021extracting} 
 & 10.2 & 11.3 & 11.6 & 11.3 & 11.3 & 10.2 & 8.5 & 9.9 & 15.5 & 14.8 & 11.4 & 11.5
 \\ 
 & Zlib \cite{carlini2021extracting} 
 & 14.4 & 16.5 & 16.2 & 15.8 & 10.6 & 17.6 & 13.4 & 14.1 & 17.3 & 19.0 & 14.4 & 16.6
 \\ 
 & Min-K\% \cite{shi2023detecting} 
 & 18.3 & 9.9 & 19.0 & 12.7 & 23.6 & 12.3 & 17.3 & 11.3 & 21.8 & 13.7 & 20.0 & 12.0
 \\ 
 & Min-K\%++ \cite{zhang2024min}
 & 12.7 & 8.1 & 16.2 & 12.7 & 18.0 & 13.4 & 16.9 & 7.0 & 24.6 & 12.3 & 17.7 & 10.7
 \\  
 & Normalized Temp
 & 18.7 & 11.6 & 27.1 & 20.4 & 20.4 & 12.0 & 16.5 & 9.2 & 27.8 & 16.9 & 22.1 & 14.0
 \\
 & Temp - Original
 & 17.6 & 12.7 & 27.5 & 13.7 & 25.7 & 12.0 & 19.0 & 12.0 & 28.2 & 21.8 & 23.6 & 14.4
 \\
\midrule

\multirow{9}{*}{128} 
 & Loss \cite{yeom2018privacy} 
 & 9.4 & 14.4 & 14.4 & 16.5 & 15.8 & 19.4 & 17.3 & 15.8 & 15.1 & 20.9 & 14.4 & 17.4
 \\ 
 & Ref \cite{carlini2021extracting} 
 & 10.1 & 7.2 & 13.7 & 8.6 & 10.1 & 5.8 & 12.9 & 12.2 & 15.8 & 18.0 & 12.5 & 10.4
 \\ 
 & Lowercase \cite{carlini2021extracting} 
 & 10.8 & 8.6 & 12.9 & 11.5 & 11.5 & 10.1 & 9.4 & 7.2 & 16.5 & 14.4 & 12.2 & 10.4
 \\ 
 & Zlib \cite{carlini2021extracting} 
 & 18.7 & 16.5 & 20.9 & 20.9 & 24.5 & 19.4 & 20.9 & 18.7 & 22.3 & 21.6 & 21.5 & 19.4
 \\ 
 & Min-K\% \cite{shi2023detecting} 
 & 13.7 & 12.2 & 18.0 & 16.5 & 18.0 & 14.4 & 19.4 & 11.5 & 26.6 & 18.7 & 19.1 & 14.7
 \\ 
 & Min-K\%++ \cite{zhang2024min}
 & 13.7 & 11.5 & 20.9 & 16.5 & 26.6 & 20.9 & 18.0 & 18.0 & 18.7 & 19.4 & 19.6 & 17.3
 \\  
 & Normalized Temp
 & 14.4 & 12.2 & 22.3 & 20.1 & 28.1 & 20.9 & 17.3 & 15.1 & 21.6 & 23.0 & 20.7 & 18.3
 \\
 & Temp - Original
 & 15.1 & 12.9 & 19.4 & 18.7 & 21.6 & 17.3 & 22.3 & 17.3 & 37.4 & 25.9 & 23.2 & 18.4
 \\
\midrule

\multirow{8}{*}{256} 
 & Loss \cite{yeom2018privacy} 
 & 3.9 & - & 5.9 & - & 5.9 & - & 9.8 & - & 13.7 & - & 7.8 & -
 \\ 
 & Ref \cite{carlini2021extracting} 
 & 3.9 & - & 5.9 & - & 5.9 & - & 3.9 & - & 2.0 & - & 4.3 & -
 \\ 
 & Lowercase \cite{carlini2021extracting} 
 & 2.0 & - & 3.9 & - & 7.8 & - & 9.8 & - & 3.9 & - & 5.5 & -
 \\ 
 & Zlib \cite{carlini2021extracting} 
 & 19.6 & - & 27.5 & - & 21.6 & - & 21.6 & - & 25.5 & - & 23.2 & -
 \\ 
 & Min-K\% \cite{shi2023detecting} 
 & 7.8 & - & 13.7 & - & 11.8 & - & 11.8 & - & 23.5 & - & 13.7 & -
 \\ 
 & Min-K\%++ \cite{zhang2024min}
 & 3.9 & - & 5.9 & - & 9.8 & - & 25.5 & - & 9.8 & - & 11.0 & -
 \\  
 & Normalized Temp
 & 19.6 & - & 17.6 & - & 7.8 & - & 31.4 & - & 11.8 & - & 17.6 & -
 \\
 & Temp - Original
 & 7.8 & - & 19.6 & - & 17.6 & - & 23.5 & - & 11.8 & - & 16.1 & -
 \\
\bottomrule


\end{tabular}
}

\end{table*}

==> tables_bold/mimir_auroc.tex <==
\begin{table*}[b]
\caption{AUROC results on the challenging MIMIR benchmark \protect\cite{duan2024membership} with non-member sets at $\le 80\%$ 13-gram overlap threshold with a suite of Pythia models \protect\cite{biderman2024emergent}.  In each column, the best result across all methods is \textbf{bolded}, with the runner-up \underline{underlined}.
% Despite not requiring a reference model like the Ref method does, our methods (NormAR and AR) consistently achieves superior or comparable performance
}
\label{tab:mimir_auroc_80}
\begin{center} \scriptsize
\setlength{\tabcolsep}{0.7pt}
\begin{tabularx}{\textwidth}{l *{20}{>{\centering\arraybackslash}X}@{}}
\toprule
\multirow{2}{*}{}  & \multicolumn{5}{c}{\textbf{Wikipedia}} & \multicolumn{5}{c}{\textbf{Github}} & \multicolumn{5}{c}{\textbf{Pile CC}} & \multicolumn{5}{c}{\textbf{PubMed Central}} \\
\cmidrule(lr){2-6}  \cmidrule(lr){7-11} \cmidrule(lr){12-16} \cmidrule(lr){17-21}
\textbf{Method}
& 160M & 1.4B & 2.8B & 6.9B & 12B
& 160M & 1.4B & 2.8B & 6.9B & 12B
& 160M & 1.4B & 2.8B & 6.9B & 12B
& 160M & 1.4B & 2.8B & 6.9B & 12B
\\
\midrule

Loss \cite{yeom2018privacy}
& 50.2 & 51.3 & 51.8 & 52.8 & 53.3 & 65.7 & 69.8 & 71.3 & 73.0 & 73.9 & 49.6 & 50.0 & 50.1 & 50.7 & 51.0 & 49.9 & 49.8 & 49.9 & 50.6 & 51.2
\\
Ref \cite{carlini2021extracting}
& \textbf{51.2} & \textbf{55.2} & \textbf{58.1} & \textbf{61.8} & \textbf{63.0} & 64.0 & 67.1 & 65.4 & 64.4 & 63.9 & 49.2 & \underline{52.2} & \textbf{53.7} & \textbf{54.9} & \textbf{56.7} & \textbf{51.3} & \textbf{53.1} & \textbf{53.7} & \textbf{55.9} & \textbf{58.0}
\\
Lowercase \cite{carlini2021extracting}
& 50.1 & 51.3 & 51.7 & 53.5 & 53.8 & 67.2 & \underline{70.3} & 71.3 & 72.9 & 73.6 & 47.8 & 48.6 & 49.5 & 50.1 & 50.4 & 49.5 & 50.4 & 51.5 & 51.5 & 52.6
\\
Zlib \cite{carlini2021extracting}
& \underline{51.1} & 52.0 & 52.4 & 53.5 & 54.1 & \textbf{67.5} & \textbf{71.0} & \textbf{72.3} & \textbf{73.9} & \textbf{74.7} & 49.6 & 50.1 & 50.3 & 50.8 & 51.1 & 49.9 & 50.0 & 50.1 & 50.6 & 51.0
\\
Min-K\% \cite{shi2023detecting}
& 50.2 & 51.3 & 51.8 & 53.6 & 54.2 & 65.7 & 69.9 & 71.4 & 73.2 & 74.2 & 50.3 & 51.0 & 50.8 & 51.5 & 51.6 & 50.6 & 50.3 & 50.5 & 51.2 & 52.1
\\
Min-K\%++ \cite{zhang2024min}
& 49.7 & \underline{53.7} & \underline{55.1} & \underline{58.0} & \underline{59.9} & 64.8 & 69.6 & 70.9 & 72.8 & 73.7 & 50.6 & 51.0 & 51.0 & 53.0 & 53.0 & 50.6 & 51.4 & 52.4 & 54.2 & 55.0
\\
NormAR (ours)
& 50.9 & 53.6 & \underline{55.1} & \underline{58.0} & \underline{59.9} & 65.8 & 69.1 & 70.1 & 72.1 & 72.9 & \textbf{52.1} & 51.8 & 52.0 & 53.4 & 53.3 & \underline{51.1} & \underline{51.7} & 52.5 & 54.2 & 55.0
\\
AR (ours)
& 50.3 & 52.9 & 54.1 & 57.1 & 59.1 & \underline{66.0} & 70.0 & \underline{71.6} & \underline{73.6} & \underline{74.4} & \underline{51.8} & \textbf{52.5} & \underline{52.6} & \underline{54.1} & \underline{54.0} & 50.9 & \underline{51.7} & \underline{52.9} & \underline{54.4} & \underline{55.2}
\\

\vspace{-.6em} \\

\toprule
\multirow{2}{*}{}  & \multicolumn{5}{c}{\textbf{ArXiv}} & \multicolumn{5}{c}{\textbf{DM Mathematics}} & \multicolumn{5}{c}{\textbf{HackerNews}} & \multicolumn{5}{c}{\textbf{Average}}\\
\cmidrule(lr){2-6}  \cmidrule(lr){7-11} \cmidrule(lr){12-16} \cmidrule(lr){17-21}
\textbf{Method} 
& 160M & 1.4B & 2.8B & 6.9B & 12B
& 160M & 1.4B & 2.8B & 6.9B & 12B
& 160M & 1.4B & 2.8B & 6.9B & 12B
& 160M & 1.4B & 2.8B & 6.9B & 12B
\\
\midrule

Loss \cite{yeom2018privacy} 
& \underline{51.0} & 51.5 & 51.9 & 52.9 & 53.3 & 48.8 & 48.5 & 48.4 & 48.5 & 48.5 & 49.4 & 50.5 & 51.3 & 52.1 & 52.6 & 52.1 & 53.1 & 53.5 & 54.4 & 54.8
\\
Ref \cite{carlini2021extracting} 
& 49.4 & 51.5 & 53.1 & \textbf{55.8} & 57.1 & 51.1 & 51.1 & 50.5 & 51.1 & 50.9 & 49.1 & \textbf{52.2} & \textbf{55.1} & \textbf{57.9} & \textbf{59.6} & 52.2 & \textbf{54.6} & \textbf{55.7} & \textbf{57.4} & \textbf{58.5}
\\
Lowercase \cite{carlini2021extracting}
& 50.8 & 50.7 & 51.3 & 51.9 & 52.3 & 48.9 & 49.0 & 49.0 & 49.1 & 48.1 & 49.0 & 50.4 & 51.1 & 51.6 & 52.1 & 51.9 & 53.0 & 53.6 & 54.4 & 54.7
\\
Zlib \cite{carlini2021extracting}
& 50.1 & 50.9 & 51.3 & 52.2 & 52.5 & 48.1 & 48.2 & 48.0 & 48.1 & 48.0 & 49.7 & 50.3 & 50.8 & 51.2 & 51.5 & 52.3 & 53.2 & 53.6 & 54.3 & 54.7
\\
Min-K\% \cite{shi2023detecting}
& \underline{51.0} & \textbf{51.7} & 52.5 & 53.6 & 54.4 & 49.4 & 49.7 & 49.5 & 49.6 & 49.7 & \underline{50.9} & 51.3 & \underline{52.6} & 53.6 & 54.5 & 52.6 & 53.6 & 54.2 & 55.2 & 55.8
\\
Min-K\%++ \cite{zhang2024min}
& 50.1 & 51.1 & 53.7 & 55.2 & \textbf{57.6} & 50.5 & 50.9 & 51.7 & 51.6 & 52.0 & 50.7 & 51.3 & \underline{52.6} & \underline{54.5} & \underline{56.3} & 52.4 & 54.1 & 55.3 & 57.0 & 58.2
\\
NormAR (ours)
& 50.9 & \underline{51.6} & \textbf{54.4} & \underline{55.6} & \textbf{57.6} & \textbf{51.8} & \textbf{52.3} & \textbf{52.8} & \textbf{53.5} & \textbf{52.4} & \textbf{51.1} & 50.7 & 52.5 & 54.3 & \underline{56.3} & \textbf{53.4} & \underline{54.4} & \underline{55.6} & \underline{57.3} & 58.2
\\
AR (ours)
& \textbf{51.4} & \textbf{51.7} & \underline{53.9} & \textbf{55.8} & \underline{57.4} & \underline{51.6} & \underline{51.7} & \underline{51.9} & \underline{52.0} & \underline{52.2} & 49.9 & 50.5 & 52.1 & 53.9 & 55.8 & \underline{53.1} & \underline{54.4} & \underline{55.6} & \underline{57.3} & \underline{58.3}
\\

\bottomrule
\end{tabularx}
\end{center}
% \vskip -0.1in
\end{table*}

==> tables_bold/mimir_auroc_13_0_2.tex <==
\begin{table*}[b]
    \caption{AUROC results on the challenging MIMIR benchmark \protect\cite{duan2024membership} with non-member sets at $\le 20\%$ 13-gram overlap threshold with a suite of Pythia models \protect\cite{biderman2024emergent}. In each column, the best result across all methods is \textbf{bolded}, with the runner-up \underline{underlined}.
    }
    \label{tab:mimir_auroc_13}
    \begin{center} \scriptsize
    \setlength{\tabcolsep}{0.7pt}
    \begin{tabularx}{\textwidth}{l *{20}{>{\centering\arraybackslash}X}@{}}
        \toprule
        \multirow{2}{*}{}  & \multicolumn{5}{c}{\textbf{Wikipedia}} & \multicolumn{5}{c}{\textbf{Github}} & \multicolumn{5}{c}{\textbf{Pile CC}} & \multicolumn{5}{c}{\textbf{PubMed Central}} \\
        \cmidrule(lr){2-6}  \cmidrule(lr){7-11} \cmidrule(lr){12-16} \cmidrule(lr){17-21}
        \textbf{Method}
        & 160M & 1.4B & 2.8B & 6.9B & 12B
        & 160M & 1.4B & 2.8B & 6.9B & 12B
        & 160M & 1.4B & 2.8B & 6.9B & 12B
        & 160M & 1.4B & 2.8B & 6.9B & 12B
        \\
        \midrule
        
    Loss \cite{yeom2018privacy}
    & 51.2 & 53.4 & 54.1 & 55.6 & 56.3 & 76.3 & 80.2 & 81.4 & 82.7 & 83.5 & 50.1 & 51.0 & 51.2 & 52.1 & 52.6 & 50.9 & 52.1 & 52.7 & 53.4 & 53.8
    \\
    Ref \cite{carlini2021extracting}
    & 50.2 & \textbf{57.1} & \textbf{59.9} & \textbf{65.1} & \textbf{66.7} & 70.5 & 74.6 & 71.6 & 70.2 & 69.5 & \textbf{50.5} & \textbf{55.0} & \textbf{56.3} & \textbf{58.7} & \textbf{60.3} & 48.9 & \textbf{54.1} & \textbf{56.1} & \textbf{58.6} & \textbf{59.4}
    \\
    Lowercase \cite{carlini2021extracting}
    & 50.9 & 53.9 & 54.4 & 56.4 & 56.9 & \textbf{79.8} & \underline{81.6} & \underline{82.4} & \underline{83.8} & \underline{84.4} & 50.6 & 51.5 & 52.3 & 53.3 & 54.5 & \textbf{52.2} & \textbf{54.1} & \underline{54.6} & 55.3 & 55.4
    \\
    Zlib \cite{carlini2021extracting}
    & 50.4 & 53.1 & 54.0 & 55.7 & 56.5 & 79.7 & \textbf{82.9} & \textbf{83.9} & \textbf{85.0} & \textbf{85.7} & 51.1 & 52.1 & 52.3 & 53.2 & 53.5 & \underline{51.5} & 52.6 & 53.1 & 53.7 & 54.0
    \\
    Min-K\% \cite{shi2023detecting}
    & 51.2 & 53.6 & 54.7 & 57.0 & 57.8 & 76.3 & 80.2 & 81.4 & 82.8 & 83.5 & 50.9 & 51.8 & 52.3 & 53.0 & 53.2 & 51.4 & 52.6 & 53.0 & 53.9 & 54.6
    \\
    Min-K\%++ \cite{zhang2024min}
    & 51.7 & \underline{55.4} & \underline{57.0} & \underline{60.4} & \underline{61.7} & 73.7 & 78.4 & 79.8 & 81.2 & 82.1 & 51.5 & 53.5 & 53.2 & 54.9 & \underline{55.3} & 50.7 & 52.7 & 53.4 & 55.2 & 55.4
    \\
    NormAR (ours)
    & \textbf{52.1} & 55.1 & 56.6 & 60.0 & 61.4 & \underline{77.2} & 78.3 & 79.7 & 81.3 & 82.2 & 51.5 & 53.5 & 53.1 & 54.8 & \underline{55.3} & 51.4 & 52.6 & 53.4 & 54.9 & 55.2
    \\
    AR (ours)
    & \underline{52.0} & 55.0 & 56.3 & 59.7 & 61.4 & 76.1 & 80.0 & 81.3 & 82.7 & 83.5 & 51.6 & 54.1 & 53.5 & 55.1 & \underline{55.3} & 51.0 & \underline{52.8} & 53.7 & \underline{55.4} & \underline{56.0}
    \\
    
            \vspace{-.6em} \\
        
        \toprule
        \multirow{2}{*}{}  & \multicolumn{5}{c}{\textbf{ArXiv}} & \multicolumn{5}{c}{\textbf{DM Mathematics}} & \multicolumn{5}{c}{\textbf{HackerNews}} & \multicolumn{5}{c}{\textbf{Average}}\\
        \cmidrule(lr){2-6}  \cmidrule(lr){7-11} \cmidrule(lr){12-16} \cmidrule(lr){17-21}
        \textbf{Method} 
        & 160M & 1.4B & 2.8B & 6.9B & 12B
        & 160M & 1.4B & 2.8B & 6.9B & 12B
        & 160M & 1.4B & 2.8B & 6.9B & 12B
        & 160M & 1.4B & 2.8B & 6.9B & 12B
        \\
        \midrule
    
    Loss \cite{yeom2018privacy} 
    & \underline{54.6} & \underline{55.8} & \underline{56.4} & 57.5 & 57.8 & \textbf{67.8} & \underline{67.5} & \underline{67.2} & \underline{67.3} & \underline{67.4} & 50.5 & \underline{51.8} & 52.6 & 53.4 & 54.0 & 57.3 & 58.8 & 59.4 & 60.3 & 60.8
    \\
    Ref \cite{carlini2021extracting} 
    & 50.3 & 54.9 & 56.3 & \textbf{59.1} & \underline{59.9} & 53.8 & 47.2 & 45.1 & 44.9 & 44.6 & 49.1 & 52.3 & \textbf{55.1} & \textbf{58.2} & \textbf{60.2} & 53.3 & 56.5 & 57.2 & 59.3 & 60.1
    \\
    Lowercase \cite{carlini2021extracting}
    & 53.7 & 54.2 & 55.2 & 55.8 & 56.7 & 56.5 & 56.6 & 58.6 & 58.0 & 56.7 & 49.3 & 50.6 & 51.5 & 52.1 & 52.3 & 56.1 & 57.5 & 58.4 & 59.2 & 59.6
    \\
    Zlib \cite{carlini2021extracting}
    & 54.2 & 55.3 & 55.7 & 56.7 & 57.0 & 64.6 & 64.7 & 64.6 & 64.6 & 64.6 & \textbf{51.2} & \textbf{51.9} & 52.4 & 52.9 & 53.2 & 57.5 & \underline{58.9} & 59.4 & 60.3 & 60.6
    \\
    Min-K\% \cite{shi2023detecting}
    & \underline{54.6} & \underline{55.8} & \underline{56.4} & 57.5 & 58.2 & \textbf{67.8} & \underline{67.5} & \underline{67.2} & \underline{67.3} & \underline{67.4} & \textbf{51.2} & 52.1 & \underline{53.4} & 54.4 & 55.1 & \underline{57.6} & 59.1 & 59.8 & 60.8 & 61.4
    \\
    Min-K\%++ \cite{zhang2024min}
    & 52.1 & 54.4 & \underline{56.4} & 57.7 & \textbf{60.1} & 59.2 & 58.6 & 59.9 & 59.4 & 59.5 & \underline{51.1} & 51.6 & 53.1 & \underline{55.0} & \underline{56.3} & 55.7 & 57.8 & 59.0 & 60.5 & 61.5
    \\
    NormAR (ours)
    & \textbf{54.8} & 55.7 & 56.1 & 57.2 & 59.6 & 65.5 & 65.3 & 65.1 & 65.7 & 64.7 & \textbf{51.2} & 51.7 & 53.1 & 54.8 & 56.1 & \textbf{57.7} & \underline{58.9} & \underline{59.6} & \underline{61.2} & \underline{62.1}
    \\
    AR (ours)
    & \underline{54.6} & \textbf{56.0} & \textbf{56.9} & \underline{58.5} & 59.8 & \underline{67.7} & \textbf{68.5} & \textbf{68.0} & \textbf{68.4} & \textbf{68.3} & 50.7 & 51.7 & 52.8 & 54.4 & 55.9 & \textbf{57.7} & \textbf{59.7} & \textbf{60.4} & \textbf{62.0} & \textbf{62.9}
    \\
        
        \bottomrule
    \end{tabularx}
    \end{center}
    % \vskip -0.1in
\end{table*}

==> tables_bold/mimir_auroc_7_0_2.tex <==
\begin{table*}[t]
    \caption{AUROC results on the challenging MIMIR benchmark \protect\cite{duan2024membership} with non-member sets at $\le 20\%$ 7-gram overlap threshold with a suite of Pythia models \protect\cite{biderman2024emergent}. In each column, the best result across all methods is \textbf{bolded}, with the runner-up \underline{underlined}.  Despite not requiring a reference model like the Ref method does, our methods (NormAR and AR) consistently achieve superior or comparable performance.\\
    }
    \label{tab:mimir_auroc}
    \vspace{-0.6cm}
    \begin{center} \scriptsize
    \setlength{\tabcolsep}{0.7pt}
    \begin{tabularx}{\textwidth}{l *{20}{>{\centering\arraybackslash}X}@{}}
        \toprule
        \multirow{2}{*}{}  & \multicolumn{5}{c}{\textbf{Wikipedia}} & \multicolumn{5}{c}{\textbf{Github}} & \multicolumn{5}{c}{\textbf{Pile CC}} & \multicolumn{5}{c}{\textbf{PubMed Central}} \\
        \cmidrule(lr){2-6}  \cmidrule(lr){7-11} \cmidrule(lr){12-16} \cmidrule(lr){17-21}
        \textbf{Method}
        & 160M & 1.4B & 2.8B & 6.9B & 12B
        & 160M & 1.4B & 2.8B & 6.9B & 12B
        & 160M & 1.4B & 2.8B & 6.9B & 12B
        & 160M & 1.4B & 2.8B & 6.9B & 12B
        \\
        \midrule
        
    Loss \cite{yeom2018privacy}
    & \underline{62.6} & 65.6 & 66.3 & 67.9 & 68.7 & 84.2 & \underline{87.3} & 88.0 & 88.9 & 89.5 & 53.3 & 54.5 & 55.0 & 56.1 & 56.5 & \underline{79.3} & 78.5 & 78.1 & 78.2 & 78.0
    \\
    Ref \cite{carlini2021extracting}
    & 53.7 & 65.1 & \textbf{68.1} & \textbf{72.4} & \textbf{73.9} & 71.5 & 78.6 & 73.4 & 70.7 & 70.0 & 51.1 & \textbf{56.3} & \textbf{58.3} & \textbf{60.8} & \textbf{61.9} & 68.5 & 67.9 & 62.9 & 62.4 & 60.0
    \\
    Lowercase \cite{carlini2021extracting}
    & 61.8 & 64.4 & 64.8 & 66.9 & 67.3 & 83.4 & 86.0 & 86.9 & 88.1 & 89.1 & 50.5 & 53.5 & 54.8 & 56.1 & 57.0 & 72.0 & 73.2 & 72.4 & 72.8 & 72.3
    \\
    Zlib \cite{carlini2021extracting}
    & 57.2 & 61.8 & 63.0 & 64.9 & 65.9 & \textbf{87.9} & \textbf{90.0} & \textbf{90.7} & \textbf{91.4} & \textbf{91.7} & 51.5 & 53.2 & 53.7 & 54.8 & 55.1 & 78.0 & 77.4 & 77.1 & 77.3 & 77.1
    \\
    Min-K\% \cite{shi2023detecting}
    & \underline{62.6} & \underline{65.8} & 66.5 & 68.4 & 69.5 & 84.2 & \underline{87.3} & \underline{88.1} & \underline{89.0} & 89.6 & 53.4 & 54.6 & 55.0 & 56.4 & 56.6 & \textbf{79.7} & \textbf{79.4} & \textbf{78.9} & \textbf{79.3} & \textbf{79.1}
    \\
    Min-K\%++ \cite{zhang2024min}
    & 59.5 & 64.4 & 65.4 & 68.9 & 70.4 & 77.8 & 83.9 & 85.4 & 86.0 & 87.3 & 52.4 & 53.3 & 54.5 & 56.4 & 56.6 & 66.5 & 68.5 & 68.6 & 70.2 & 69.8
    \\
    Norm AR (ours)
    & 61.5 & 64.5 & 65.3 & 68.9 & 70.4 & \underline{84.3} & 85.7 & 86.6 & 87.8 & 88.5 & \textbf{53.5} & \underline{55.8} & \underline{56.2} & \underline{56.8} & \underline{57.1} & 75.7 & 76.9 & 76.7 & 77.2 & 76.1
    \\
    AR (ours)
    & \textbf{62.7} & \textbf{66.1} & \underline{67.0} & \underline{69.9} & \underline{71.5} & 84.0 & 87.1 & 88.0 & \underline{89.0} & \underline{89.7} & \underline{53.4} & 55.1 & 55.5 & 56.7 & 57.0 & \underline{79.3} & \underline{78.6} & \underline{78.3} & \underline{78.7} & \underline{78.2}
    \\
    
            \vspace{-.6em} \\
        
        \toprule
        \multirow{2}{*}{}  & \multicolumn{5}{c}{\textbf{ArXiv}} & \multicolumn{5}{c}{\textbf{DM Mathematics}} & \multicolumn{5}{c}{\textbf{HackerNews}} & \multicolumn{5}{c}{\textbf{Average}}\\
        \cmidrule(lr){2-6}  \cmidrule(lr){7-11} \cmidrule(lr){12-16} \cmidrule(lr){17-21}
        \textbf{Method} 
        & 160M & 1.4B & 2.8B & 6.9B & 12B
        & 160M & 1.4B & 2.8B & 6.9B & 12B
        & 160M & 1.4B & 2.8B & 6.9B & 12B
        & 160M & 1.4B & 2.8B & 6.9B & 12B
        \\
        \midrule
    
    Loss \cite{yeom2018privacy} 
    & \underline{75.6} & \underline{77.6} & \underline{78.1} & \underline{79.1} & \underline{79.5} & 93.7 & 92.2 & 91.9 & 92.0 & 91.9 & 58.6 & \underline{59.7} & \textbf{60.6} & \textbf{61.3} & 61.9 & \underline{72.5} & 73.6 & 74.0 & 74.8 & 75.1
    \\
    Ref \cite{carlini2021extracting} 
    & 61.8 & 70.8 & 71.0 & 73.2 & 74.2 & 64.1 & 47.6 & 43.8 & 43.5 & 42.9 & 52.3 & 55.0 & 57.3 & 59.8 & \textbf{62.6} & 60.4 & 63.0 & 62.1 & 63.3 & 63.6
    \\
    Lowercase \cite{carlini2021extracting}
    & 70.3 & 72.5 & 73.7 & 74.6 & 74.8 & 86.1 & 85.3 & 92.8 & 92.8 & 90.3 & 51.0 & 52.3 & 54.0 & 54.1 & 54.8 & 67.9 & 69.6 & 71.3 & 72.2 & 72.2
    \\
    Zlib \cite{carlini2021extracting}
    & 75.1 & 77.1 & 77.5 & 78.4 & 78.7 & 81.2 & 80.8 & 81.1 & 81.3 & 81.2 & 57.7 & 58.7 & 59.4 & 59.8 & 60.3 & 69.8 & 71.3 & 71.8 & 72.6 & 72.9
    \\
    Min-K\% \cite{shi2023detecting}
    & \underline{75.6} & \underline{77.6} & \underline{78.1} & \underline{79.1} & \underline{79.5} & \underline{93.8} & 92.9 & 93.2 & 93.1 & 93.1 & \underline{58.7} & \underline{59.7} & \textbf{60.6} & \textbf{61.3} & 62.0 & \textbf{72.6} & \underline{73.9} & \underline{74.3} & \underline{75.2} & \underline{75.6}
    \\
    Min-K\%++ \cite{zhang2024min}
    & 60.6 & 65.8 & 67.3 & 70.0 & 71.6 & 83.0 & 75.8 & 79.1 & 77.5 & 78.3 & 55.3 & 56.8 & 58.6 & 59.9 & 61.1 & 65.0 & 66.9 & 68.4 & 69.8 & 70.7
    \\
    NormAR (ours)
    & \textbf{77.1} & \textbf{77.7} & \textbf{78.5} & 79.0 & 79.1 & 93.6 & \textbf{94.4} & \underline{93.9} & \underline{94.3} & \underline{94.9} & \textbf{59.6} & \textbf{60.0} & \underline{60.4} & \underline{60.7} & 61.2 & 72.2 & 73.6 & 73.9 & 75.0 & 75.3
    \\
    AR (ours)
    & \underline{75.6} & \underline{77.6} & \underline{78.1} & \textbf{79.2} & \textbf{79.6} & \textbf{94.5} & \underline{94.2} & \textbf{94.3} & \textbf{95.1} & \textbf{95.5} & 58.6 & 59.6 & \textbf{60.6} & \textbf{61.3} & \underline{62.2} & \textbf{72.6} & \textbf{74.0} & \textbf{74.5} & \textbf{75.7} & \textbf{76.2}
    \\
        
        \bottomrule
    \end{tabularx}
    \end{center}
    \vspace{-0.5cm}
    \end{table*}

==> tables_bold/mimir_tpr.tex <==
\begin{table*}[b]
\caption{TPR at low FPR (FPR=5\%) results on the challenging MIMIR benchmark \protect\cite{duan2024membership} with non-member sets at $\le 80\%$ 13-gram overlap threshold with a suite of Pythia models \protect\cite{biderman2024emergent}.  In each column, the best result across all methods is \textbf{bolded}, with the runner-up \underline{underlined}.
}
\label{tab:mimir_tpr}
\begin{center} \scriptsize
\setlength{\tabcolsep}{0.7pt}
\begin{tabularx}{\textwidth}{l *{20}{>{\centering\arraybackslash}X}@{}}
\toprule
\multirow{2}{*}{}  & \multicolumn{5}{c}{\textbf{Wikipedia}} & \multicolumn{5}{c}{\textbf{Github}} & \multicolumn{5}{c}{\textbf{Pile CC}} & \multicolumn{5}{c}{\textbf{PubMed Central}} \\
\cmidrule(lr){2-6}  \cmidrule(lr){7-11} \cmidrule(lr){12-16} \cmidrule(lr){17-21}
\textbf{Method}
& 160M & 1.4B & 2.8B & 6.9B & 12B
& 160M & 1.4B & 2.8B & 6.9B & 12B
& 160M & 1.4B & 2.8B & 6.9B & 12B
& 160M & 1.4B & 2.8B & 6.9B & 12B
\\
\midrule

Loss \cite{yeom2018privacy} 
& 4.2 & 4.7 & 4.7 & 5.1 & 5.0 & 22.6 & 32.1 & 33.6 & \underline{38.5} & 40.7 & 3.1 & 5.0 & 4.8 & 4.9 & 5.4 & 4.0 & 4.4 & 4.3 & 4.9 & 5.1
\\
Ref \cite{carlini2021extracting} 
& \textbf{6.1} & 5.3 & 5.5 & 5.6 & 5.5 & 23.4 & 14.8 & 14.9 & 15.4 & 16.5 & 5.5 & \textbf{5.6}& \underline{5.8} & 5.8 & \textbf{7.4}& \textbf{5.7} & 4.1 & 4.0 & 5.9 & \underline{7.3}
\\
Lowercase \cite{carlini2021extracting}
& 4.6 & 4.5 & 4.9 & 5.2 & 5.5 & 24.4 & 32.2 & 34.3 & 38.1 & 38.0 & 3.4 & 5.3 & 5.3 & \underline{6.2} & 6.3 & 3.5 & 5.0 & 5.3 & 6.0 & 4.9
\\
Zlib \cite{carlini2021extracting}
& 4.2 & 5.7 & 5.9 & 6.3 & 6.6 & \underline{25.0} & \underline{32.8} & \textbf{36.1} & \textbf{40.1} & \underline{40.8} & 4.0 & \underline{5.1} & 5.4 & \underline{6.2} & 6.6 & 3.8 & 3.6 & 3.5 & 4.3 & 4.4
\\
Min-K\% \cite{shi2023detecting}
& 4.2 & 4.7 & 5.2 & 6.5 & 8.1 & 22.6 & 31.9 & 34.0 & 39.0 & 39.5 & 4.2 & 4.4 & 3.9 & 4.4 & 4.9 & 4.7 & 4.6 & 4.5 & 5.1 & 5.4
\\
Min-K\%++ \cite{zhang2024min}
& \underline{5.3} & \underline{5.8} & \textbf{8.5} & \textbf{11.4} & \underline{10.2} & \underline{25.0} & \textbf{33.0} & 34.2 & 38.2 & 40.0 & 4.7 & 5.0 & 4.8 & 6.0 & 5.7 & 3.9 & \textbf{6.3} & \textbf{6.5} & \textbf{7.4} & \textbf{8.4}
\\
NormAR (ours)
& 4.3 & \underline{5.8} & \textbf{8.5} & \textbf{11.4} & \underline{10.2} & \textbf{25.5} & 31.6 & 33.1 & 36.1 & 38.4 & \textbf{6.2} & 4.7 & 4.3 & 6.0 & 5.1 & 4.9 & \underline{5.8} & \underline{6.0} & \underline{6.9} & \textbf{8.4}
\\
AR (ours)
& \underline{5.3} & \textbf{6.1} & \underline{8.0} & \underline{10.3} & \textbf{11.0} & 24.2 & 32.4 & \underline{34.4} & 37.4 & \textbf{42.2} & \underline{5.8} & 4.9 & \textbf{6.4} & \textbf{7.1} & \underline{7.0} & \underline{5.6} & 5.4 & 4.9 & 6.0 & 6.2
\\

\vspace{-.6em} \\

\toprule
\multirow{2}{*}{}  & \multicolumn{5}{c}{\textbf{ArXiv}} & \multicolumn{5}{c}{\textbf{DM Mathematics}} & \multicolumn{5}{c}{\textbf{HackerNews}} & \multicolumn{5}{c}{\textbf{Average}}\\
\cmidrule(lr){2-6}  \cmidrule(lr){7-11} \cmidrule(lr){12-16} \cmidrule(lr){17-21}
\textbf{Method} 
& 160M & 1.4B & 2.8B & 6.9B & 12B
& 160M & 1.4B & 2.8B & 6.9B & 12B
& 160M & 1.4B & 2.8B & 6.9B & 12B
& 160M & 1.4B & 2.8B & 6.9B & 12B
\\
\midrule

Loss \cite{yeom2018privacy} 
& 4.0 & 4.8 & 4.6 & 5.4 & 5.9 & 3.8 & 4.3 & 4.1 & 4.1 & 4.2 & 5.0 & 4.8 & 5.5 & 5.9 & 6.4 & 6.7 & 8.6 & 8.8 & 9.8 & 10.4
\\
Ref \cite{carlini2021extracting} 
& \underline{5.2} & 5.4 & \underline{5.9} & \underline{6.8} & \textbf{7.7} & \underline{5.3} & 3.6 & 4.9 & 5.4 & \textbf{5.8} & 5.2 & \textbf{6.3} & \textbf{7.6} & \textbf{7.0} & \textbf{7.7} & \underline{8.1} & 6.4 & 6.9 & 7.4 & 8.3
\\
Lowercase \cite{carlini2021extracting}
& 5.1 & 4.7 & 5.4 & 5.6 & 5.0 & \textbf{5.6} & \underline{6.2} & \underline{5.5} & \textbf{6.8} & 5.5 & 5.2 & 5.2 & \underline{6.3} & \underline{6.6} & 6.7 & 7.4 & 9.0 & 9.6 & 10.6 & 10.3
\\
Zlib \cite{carlini2021extracting}
& 2.9 & 4.3 & 4.1 & 4.6 & 4.3 & 4.1 & 5.0 & 4.6 & 4.3 & 4.3 & 5.0 & \underline{5.5} & 5.8 & 5.6 & 5.7 & 7.0 & 8.9 & 9.3 & 10.2 & 10.4
\\
Min-K\% \cite{shi2023detecting}
& 4.0 & 3.9 & 4.2 & 4.6 & 4.8 & 4.5 & 4.1 & 4.5 & 4.5 & 4.6 & 4.9 & 5.1 & 5.9 & 6.3 & 6.2 & 7.0 & 8.4 & 8.9 & 10.1 & 10.5
\\
Min-K\%++ \cite{zhang2024min}
& 4.3 & \underline{6.0} & \textbf{6.7} & \textbf{7.4} & \textbf{7.7} & 5.1 & 5.4 & 5.3 & 6.2 & \underline{5.6} & 4.4 & 3.7 & 4.9 & 6.4 & 4.7 & 7.5 & \textbf{9.3} & \textbf{10.1} & \textbf{11.9} & \underline{11.8}
\\
NormAR (ours)
& 3.6 & \textbf{6.2} & 5.4 & 3.8 & \textbf{7.7} & 4.2 & \textbf{6.3} & \textbf{6.1} & \underline{6.5} & 5.4 & \textbf{6.7} & 4.2 & 5.6 & 4.4 & 4.7 & 7.9 & \underline{9.2} & \underline{9.9} & 10.7 & 11.4
\\
AR (ours)
& \textbf{5.3} & 4.1 & 3.7 & 4.4 & \underline{6.2} & \textbf{5.6} & 4.9 & 4.0 & 5.6 & 4.5 & 6.1 & 5.0 & 6.2 & 5.8 & \underline{7.2} & \textbf{8.3} & 9.0 & 9.7 & \underline{10.9} & \textbf{12.0}
\\

\bottomrule
\end{tabularx}
\end{center}
% \vskip -0.1in
\end{table*}

==> tables_bold/mimir_tpr_13_0_2.tex <==
\begin{table*}[b]
    \caption{TPR at low FPR (FPR=5\%) results on the challenging MIMIR benchmark \protect\cite{duan2024membership} with non-member sets at $\le 20\%$ 13-gram overlap threshold with a suite of Pythia models \protect\cite{biderman2024emergent}. In each column, the best result across all methods is \textbf{bolded}, with the runner-up \underline{underlined}.
    }
    \label{tab:mimir_tpr_13}
    \begin{center} \scriptsize
    \setlength{\tabcolsep}{0.7pt}
    \begin{tabularx}{\textwidth}{l *{20}{>{\centering\arraybackslash}X}@{}}
        \toprule
        \multirow{2}{*}{}  & \multicolumn{5}{c}{\textbf{Wikipedia}} & \multicolumn{5}{c}{\textbf{Github}} & \multicolumn{5}{c}{\textbf{Pile CC}} & \multicolumn{5}{c}{\textbf{PubMed Central}} \\
        \cmidrule(lr){2-6}  \cmidrule(lr){7-11} \cmidrule(lr){12-16} \cmidrule(lr){17-21}
        \textbf{Method}
        & 160M & 1.4B & 2.8B & 6.9B & 12B
        & 160M & 1.4B & 2.8B & 6.9B & 12B
        & 160M & 1.4B & 2.8B & 6.9B & 12B
        & 160M & 1.4B & 2.8B & 6.9B & 12B
        \\
        \midrule
        
    Loss \cite{yeom2018privacy} 
    & \textbf{7.9} & \underline{10.1} & \textbf{11.5} & 12.1 & 12.6 & 36.9 & 45.1 & 49.7 & 54.1 & 53.8 & 3.6 & 7.3 & 7.5 & 8.2 & 8.9 & 4.7 & 4.8 & 5.6 & 5.9 & 5.7
    \\
    Ref \cite{carlini2021extracting} 
    & 6.0 & 9.5 & 10.8 & 12.7 & 12.3 & 33.6 & 23.4 & 19.2 & 19.3 & 20.0 & \textbf{5.8} & \textbf{8.9} & \textbf{10.3} & \textbf{12.9} & \textbf{13.4} & 4.8 & 4.9 & 5.0 & \textbf{7.4} & \textbf{9.2}
    \\
    Lowercase \cite{carlini2021extracting}
    & 6.5 & 9.9 & 9.7 & 10.8 & 10.6 & \underline{52.4} & \underline{56.2} & \underline{57.3} & \underline{59.5} & \underline{61.4} & 5.2 & \underline{8.5} & \underline{8.2} & \underline{9.6} & \underline{10.6} & \textbf{5.2} & \textbf{6.5} & \textbf{7.1} & 6.8 & \underline{8.9}
    \\
    Zlib \cite{carlini2021extracting}
    & 7.0 & 8.6 & 9.6 & 10.2 & 10.7 & \textbf{52.8} & \textbf{57.8} & \textbf{59.9} & \textbf{62.3} & \textbf{62.7} & \underline{5.5} & 7.4 & 7.9 & 9.1 & 9.9 & 4.1 & 4.6 & 5.1 & 5.0 & 5.7
    \\
    Min-K\% \cite{shi2023detecting}
    & \textbf{7.9} & 9.3 & \textbf{11.5} & 12.1 & 12.0 & 36.9 & 45.1 & 49.9 & 54.1 & 53.8 & 4.6 & 6.2 & 5.5 & 6.2 & 6.6 & 4.3 & 5.9 & 5.7 & 6.1 & 6.7
    \\
    Min-K\%++ \cite{zhang2024min}
    & 6.9 & \textbf{10.2} & \underline{11.1} & \textbf{13.7} & \textbf{14.7} & 33.8 & 44.5 & 45.3 & 50.0 & 52.4 & 4.2 & 7.7 & 7.3 & 7.9 & 9.4 & 3.8 & \underline{6.4} & 6.4 & 6.2 & 8.5
    \\
    NormAR (ours)
    & \underline{7.2} & \underline{10.1} & 9.5 & 12.2 & 12.6 & 38.6 & 43.0 & 45.9 & 49.7 & 53.2 & 4.2 & 7.7 & 6.2 & 7.8 & 8.1 & \underline{4.8} & \underline{6.4} & 5.1 & \underline{7.2} & 7.6
    \\
    AR (ours)
    & 7.1 & \textbf{10.2} & 10.3 & \underline{13.1} & \underline{14.0} & 34.2 & 45.5 & 49.1 & 52.3 & 52.7 & 3.6 & 6.1 & 6.6 & 8.0 & 7.5 & 4.5 & 6.2 & \underline{6.9} & 7.1 & 8.2
    \\
    
            \vspace{-.6em} \\
        
        \toprule
        \multirow{2}{*}{}  & \multicolumn{5}{c}{\textbf{ArXiv}} & \multicolumn{5}{c}{\textbf{DM Mathematics}} & \multicolumn{5}{c}{\textbf{HackerNews}} & \multicolumn{5}{c}{\textbf{Average}}\\
        \cmidrule(lr){2-6}  \cmidrule(lr){7-11} \cmidrule(lr){12-16} \cmidrule(lr){17-21}
        \textbf{Method} 
        & 160M & 1.4B & 2.8B & 6.9B & 12B
        & 160M & 1.4B & 2.8B & 6.9B & 12B
        & 160M & 1.4B & 2.8B & 6.9B & 12B
        & 160M & 1.4B & 2.8B & 6.9B & 12B
        \\
        \midrule
    
    Loss \cite{yeom2018privacy} 
    & 6.8 & 7.7 & 8.1 & 8.9 & 9.8 & \underline{19.2} & 14.8 & 12.2 & 11.8 & 12.1 & 5.7 & 5.0 & 6.3 & 6.3 & 7.2 & \underline{10.6} & 9.2 & 8.9 & 9.0 & 9.7
    \\
    Ref \cite{carlini2021extracting} 
    & 5.7 & \underline{7.9} & 8.4 & 9.9 & 9.8 & 5.8 & 2.1 & 3.0 & 2.8 & 2.6 & 5.5 & 6.1 & \underline{7.7} & \underline{7.1} & \textbf{9.3} & 5.7 & 5.4 & 6.4 & 6.6 & 7.2
    \\
    Lowercase \cite{carlini2021extracting}
    & \textbf{7.9} & 7.7 & 7.5 & 9.5 & 9.3 & 10.4 & 9.5 & 9.4 & 15.3 & 10.8 & 5.0 & 5.1 & 6.5 & 6.8 & 6.8 & 7.8 & 7.4 & 7.8 & 10.5 & 9.0
    \\
    Zlib \cite{carlini2021extracting}
    & 6.4 & 7.6 & \textbf{8.8} & \underline{10.7} & \textbf{11.1} & 16.0 & 11.3 & 10.0 & 10.9 & 10.7 & \textbf{6.6} & 5.9 & 6.4 & 6.7 & 7.1 & 9.7 & 8.3 & 8.4 & 9.4 & 9.6
    \\
    Min-K\% \cite{shi2023detecting}
    & \underline{7.0} & 7.8 & 8.4 & 9.3 & 10.7 & \underline{19.2} & 14.8 & 12.2 & 12.1 & 12.2 & 5.4 & \underline{6.4} & 6.8 & 6.3 & \underline{7.9} & 10.5 & 9.7 & 9.1 & 9.2 & 10.3
    \\
    Min-K\%++ \cite{zhang2024min}
    & 6.8 & 7.2 & 8.3 & \textbf{11.0} & \underline{10.9} & 9.0 & 10.6 & 11.3 & 11.2 & 11.6 & 4.3 & 4.0 & 4.5 & 6.6 & 5.2 & 6.7 & 7.3 & 8.0 & 9.6 & 9.2
    \\
    NormAR (ours)
    & 6.0 & 7.1 & 7.9 & 10.3 & 10.4 & \underline{19.2} & \underline{16.3} & \underline{15.7} & \underline{19.7} & \underline{16.7} & 4.2 & \textbf{6.6} & 5.5 & 7.1 & 5.5 & 9.8 & \underline{10.0} & \underline{9.7} & \underline{12.4} & \underline{10.9}
    \\
    AR (ours)
    & 6.9 & \textbf{8.1} & \underline{8.7} & 10.4 & 9.9 & \textbf{21.6} & \textbf{21.0} & \textbf{19.9} & \textbf{21.4} & \textbf{20.6} & \underline{5.9} & 5.4 & \textbf{8.1} & \textbf{7.2} & 6.1 & \textbf{11.5} & \textbf{11.5} & \textbf{12.2} & \textbf{13.0} & \textbf{12.2}
    \\
        
        \bottomrule
    \end{tabularx}
    \end{center}
    % \vskip -0.1in
    \end{table*}

==> tables_bold/mimir_tpr_7_0_2.tex <==
\begin{table*}[b]
    \caption{TPR at low FPR (FPR=5\%) results on the challenging MIMIR benchmark \protect\cite{duan2024membership} with non-member sets at $\le 20\%$ 7-gram overlap threshold with a suite of Pythia models \protect\cite{biderman2024emergent}. In each column, the best result across all methods is \textbf{bolded}, with the runner-up \underline{underlined}.
}
    \label{tab:mimir_trp_0.7}
    \begin{center} \scriptsize
    \setlength{\tabcolsep}{0.7pt}
    \begin{tabularx}{\textwidth}{l *{20}{>{\centering\arraybackslash}X}@{}}
            \toprule
            \multirow{2}{*}{}  & \multicolumn{5}{c}{\textbf{Wikipedia}} & \multicolumn{5}{c}{\textbf{Github}} & \multicolumn{5}{c}{\textbf{Pile CC}} & \multicolumn{5}{c}{\textbf{PubMed Central}} \\
            \cmidrule(lr){2-6}  \cmidrule(lr){7-11} \cmidrule(lr){12-16} \cmidrule(lr){17-21}
            \textbf{Method}
            & 160M & 1.4B & 2.8B & 6.9B & 12B
            & 160M & 1.4B & 2.8B & 6.9B & 12B
            & 160M & 1.4B & 2.8B & 6.9B & 12B
            & 160M & 1.4B & 2.8B & 6.9B & 12B
            \\
            \midrule
            
        Loss \cite{yeom2018privacy} 
        & 19.6 & \underline{23.7} & 22.8 & 24.0 & 24.4 & 41.4 & 58.2 & 57.1 & 61.9 & 61.2 & 8.3 & 11.1 & 11.4 & 13.7 & 13.9 & 29.9 & 31.0 & 32.0 & 30.5 & 32.6
        \\
        Ref \cite{carlini2021extracting} 
        & 8.7 & 21.3 & 19.5 & 20.9 & 20.4 & 26.5 & 27.2 & 23.9 & 22.4 & 20.5 & 6.9 & \textbf{12.7} & \textbf{14.4} & \textbf{17.1} & \textbf{17.9} & 20.6 & 6.5 & 5.1 & 4.1 & 4.3
        \\
        Lowercase \cite{carlini2021extracting}
        & \textbf{20.7} & 21.4 & 21.5 & 22.8 & 23.9 & \underline{63.4} & \underline{67.5} & \underline{67.5} & \underline{66.0} & \underline{67.9} & 8.4 & 10.1 & 9.5 & 12.0 & 11.0 & 21.4 & 25.3 & 18.9 & 20.0 & 17.1
        \\
        Zlib \cite{carlini2021extracting}
        & 14.4 & 20.2 & 19.5 & 20.5 & 21.5 & \textbf{63.8} & \textbf{70.5} & \textbf{71.3} & \textbf{74.3} & \textbf{75.7} & \underline{9.5} & \textbf{12.7} & 12.4 & 13.9 & 14.2 & 26.7 & 29.5 & 29.3 & 29.1 & 28.1
        \\
        Min-K\% \cite{shi2023detecting}
        & 19.9 & 22.7 & \underline{23.0} & 23.7 & 26.1 & 41.4 & 58.2 & 56.0 & 61.9 & 60.4 & 8.4 & \underline{11.8} & 12.2 & \underline{14.5} & \underline{14.8} & \textbf{35.2} & \textbf{35.6} & \textbf{35.0} & \underline{34.2} & \underline{34.0}
        \\
        Min-K\%++ \cite{zhang2024min}
        & 15.7 & 19.7 & 22.4 & 23.4 & 26.0 & 36.9 & 54.1 & 54.9 & 56.0 & 58.2 & 7.0 & 10.3 & 10.9 & 12.8 & 11.4 & 20.0 & 20.4 & 21.4 & 24.8 & 22.8
        \\
        NormAR (ours)
        & 16.6 & 21.2 & 22.5 & \underline{24.4} & \underline{26.5} & 47.8 & 51.9 & 53.7 & 59.0 & 64.2 & 8.1 & 10.6 & 10.6 & 11.8 & 12.0 & 16.5 & 17.3 & 26.7 & 29.7 & 21.4
        \\
        AR (ours)
        & \underline{20.5} & \textbf{25.1} & \textbf{25.}2 & \textbf{24.9} & \textbf{28.5} & 40.3 & 54.9 & 54.1 & 57.5 & 62.7 & \textbf{9.9} & 10.9 & \underline{12.5} & 13.6 & 12.9 & \underline{31.0} & \underline{33.6} & \underline{33.8} & \textbf{34.6} & \textbf{34.6}
        \\
        
                \vspace{-.6em} \\
            
            \toprule
            \multirow{2}{*}{}  & \multicolumn{5}{c}{\textbf{ArXiv}} & \multicolumn{5}{c}{\textbf{DM Mathematics}} & \multicolumn{5}{c}{\textbf{HackerNews}} & \multicolumn{5}{c}{\textbf{Average}}\\
            \cmidrule(lr){2-6}  \cmidrule(lr){7-11} \cmidrule(lr){12-16} \cmidrule(lr){17-21}
            \textbf{Method} 
            & 160M & 1.4B & 2.8B & 6.9B & 12B
            & 160M & 1.4B & 2.8B & 6.9B & 12B
            & 160M & 1.4B & 2.8B & 6.9B & 12B
            & 160M & 1.4B & 2.8B & 6.9B & 12B
            \\
            \midrule
        
        Loss \cite{yeom2018privacy} 
        & 29.0 & \underline{32.0} & \underline{34.2} & \underline{37.0} & \underline{36.2} & 79.8 & 62.9 & 59.6 & 62.9 & 62.9 & 8.7 & \textbf{11.0} & \underline{11.6} & 12.2 & \underline{14.1} & \underline{31.0} & 32.8 & 32.7 & 34.6 & 35.0
        \\
        Ref \cite{carlini2021extracting} 
        & 10.4 & 20.4 & 19.0 & 21.8 & 22.6 & 4.5 & 4.5 & 6.7 & 5.6 & 3.4 & 5.9 & 7.4 & 8.4 & 9.8 & 11.1 & 11.9 & 14.3 & 13.9 & 14.5 & 14.3
        \\
        Lowercase \cite{carlini2021extracting}
        & 25.2 & 26.6 & 25.0 & 27.6 & 28.2 & 58.4 & 65.2 & 66.3 & 67.4 & 64.0 & 6.8 & 5.9 & 7.4 & 8.0 & 7.4 & 29.2 & 31.7 & 30.9 & 32.0 & 31.4
        \\
        Zlib \cite{carlini2021extracting}
        & 28.0 & 30.6 & \textbf{34.6} & 33.6 & 33.4 & 22.5 & 16.9 & 16.9 & 16.9 & 16.9 & \textbf{11.3} & \underline{10.7} & 10.5 & 11.8 & 12.7 & 25.2 & 27.3 & 27.8 & 28.6 & 28.9
        \\
        Min-K\% \cite{shi2023detecting}
        & 29.0 & \textbf{32.2} & \underline{34.2} & \underline{37.0} & \textbf{36.4} & 79.8 & 69.7 & 69.7 & 69.7 & 69.7 & 8.8 & \textbf{11.0} & 11.6 & 12.4 & 13.9 & 31.8 & \underline{34.5} & \underline{34.5} & 36.2 & 36.5
        \\
        Min-K\%++ \cite{zhang2024min}
        & 12.0 & 12.8 & 16.8 & 17.0 & 22.6 & 53.9 & 36.0 & 31.5 & 34.8 & 29.2 & 7.7 & 8.5 & 8.8 & 9.3 & 9.0 & 21.9 & 23.1 & 23.8 & 25.4 & 25.6
        \\
        NormAR (ours)
        & \textbf{30.4} & 29.6 & 32.8 & 34.2 & 35.0 & \underline{84.3} & \textbf{87.6} & \underline{70.8} & \underline{76.4} & \underline{82.0} & \underline{10.1} & 9.6 & \textbf{11.9} & \underline{12.5} & 11.3 & 30.5 & 32.5 & 32.7 & \underline{35.4} & \underline{36.1}
        \\
        AR (ours)
        & \underline{29.4} & \textbf{32.2} & \underline{34.2} & \textbf{40.2} & \underline{36.2} & \textbf{85.4} & \underline{75.3} & \textbf{83.1} & \textbf{84.3} & \textbf{85.4} & 9.8 & \textbf{11.0} & \textbf{11.9} & \textbf{13.2} & \textbf{14.2} & \textbf{32.3} & \textbf{34.7} & \textbf{36.4} & \textbf{38.3} & \textbf{39.2}
        \\
            
        \bottomrule
    \end{tabularx}
    \end{center}
\end{table*}

==> tables_bold/patent_wikimia_mimir_fpr.tex <==
\begin{table*}[t]
\centering
\small % font size
\setlength{\tabcolsep}{7.pt} % column separation
\renewcommand{\arraystretch}{1.1} % row space 
\begin{tabular}{l cccc cccccc cccc}
\toprule
\multirow{4}{*}{\textbf{Method}}
& \multicolumn{4}{c}{PatentMIA}
& \multicolumn{6}{c}{WikiMIA}
& \multicolumn{4}{c}{MIMIR}
\\ 
\cmidrule(r){2-5}
\cmidrule(r){6-11}
\cmidrule(r){12-15}
% \cmidrule{5-8} 
% & Baichuan-13B   & Qwen1.5-14B   & OPT-6.7B & Pythia-6.9B & Pythia-12B & OPT-13B & GPT-NeoX-20B
% & \multirow{2}{*}{\textbf{B-13B}}
% & \multirow{2}{*}{\textbf{B2-13B}}
% & \multirow{2}{*}{\textbf{Q-32B}}
% & \multirow{2}{*}{\textbf{Q-72B}}
& \multicolumn{2}{c}{\textbf{Baichuan}}
& \multicolumn{2}{c}{\textbf{Qwen1.5}}

& \multicolumn{2}{c}{\textbf{OPT-6.7B}}
% & \multicolumn{2}{c}{\textbf{Pythia-6.9B}}
& \multicolumn{2}{c}{\textbf{Pythia-12B}}
% & \multicolumn{2}{c}{\textbf{OPT-13B}}
& \multicolumn{2}{c}{\textbf{NeoX-20B}}

& \multicolumn{4}{c}{\textbf{Pythia}}
\\ 
\cmidrule(r){2-3}
\cmidrule(r){4-5}
\cmidrule(r){6-7}
\cmidrule(r){8-9}
\cmidrule(r){10-11}
\cmidrule(r){12-15}
% \cmidrule(r){12-13}
% \cmidrule(r){14-15}

& 13B & 2-13B & 32B & 72B & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} & 1.4B & 2.8B & 6.9B & 12B
\\ 
\midrule
Loss
& 16.3 & 18.6 & 17.0 & 10.8
& 12.9    & 15.1    & 15.8    & 18.7    & 20.1    & 18.0
& 41.3 & 41.1 & 43.0 & 43.7

\\
Ref
& 14.0 & 3.4 & 7.7 & 1.4
& 10.8    & 8.6    & 9.4    & 10.1    & 15.8    & 18.7
& 15.3 & 14.7 & 15.9 & 14.4

\\
Lowercase
& - & - & - & -
& 10.1    & 7.9    & 13.7    & 11.5    & 12.9    & 12.9
& 41.2 & 39.8 & 40.8 & 40.2

\\
Zlib
& 16.1 & 16.8 & 13.4 & 6.3
& 18.0    & 15.1    & 23.7    & 19.4    & 21.6    & 22.3
& 33.4 & 34.3 & 34.2 & 35.2

\\
Min-K\%
& 17.3 & 21.7 & 18.3 & 10.9
& 20.9    & 15.8    & 23.7    & 20.9    & 24.5    & 22.3
& 43.9 & 44.8 & 45.8 & 47.3

\\
Min-K\%++
& 13.6 & 17.0 & 16.1 & 14.8
& 23.7    & 21.6    & 23.0    & 22.3    & 24.5    & 18.7
& 28.5 & 30.0 & 31.2 & 31.3

\\
DC-PDD
& \textbf{28.0} & \textbf{27.4} & 22.3 & 11.0
& 19.4    & 21.6    & 25.9    & 21.6    & \textbf{30.2}    & \textbf{28.1}
& 50.5 & 51.2 & 51.2 & 51.8

\\
\hline
AC
& 23.8 & 25.8 & 29.7 & 33.0
& \textbf{33.1}    & 30.9    & 27.3    & \textbf{26.6}    & \textbf{30.2}    & 27.3
& 51.6 & 51.8 & 53.2 & 52.9

\\
DerivAC
& 25.9 & 25.2 & \textbf{30.6} & \textbf{33.6}
& \textbf{33.1}    & 30.9    & 27.3    & \textbf{26.6}    & 28.8    & 27.3
& 53.6 & \textbf{53.9} & 54.3 & \textbf{54.6}

\\
NormAC
& 26.3 & 24.3 & 24.7 & 25.7
& 30.2    & \textbf{35.3}    & \textbf{28.8}    & \textbf{26.6}    & 28.1    & 25.2
& \textbf{54.1} & 53.8 & \textbf{55.4} & 54.3

\\
\bottomrule
\end{tabular}
\caption{FPR@95\%TPR (5\%FNR) scores for evaluating MIAs across different benchmarks and LLMs. Lower scores indicate better detection of pre-training texts. We report the TPR@5\%FPR scores of our ACMIA methods, i.e., AC, DerivAC, and NormAC, with the optimal temperature. We report the average TPR@95\%TPR scores of different subsets in MIMIR.}
% More detailed results of these subsets are reported in the Appendix. \textbf{Bold} indicates the best MIA performance.

\label{tab:fpr}
\end{table*}

==> tables_bold/wiki_main_results.tex <==
\begin{table*}[t]
    \centering
    %\footnotesize
    \caption{AUROC results on the WikiMIA benchmark \protect\cite{shi2023detecting}. \textit{Ori.} and \textit{Para.} denote the original and paraphrased settings, respectively. \textbf{Bolded} and \underline{underlined} numbers indicate the best result and the runner-up within each column across all methods. The proposed ARMIA, including NormAR and AR, demonstrates significant improvements over existing methods in most settings.}


    \label{tab:wikimia_main}
    \vspace{-0.4cm}
    \resizebox{0.98\textwidth}{!}{%
    \begin{tabular}{llcccccccccccc}\\
    \toprule
    & & \multicolumn{2}{c}{\textbf{Pythia-2.8B}} & \multicolumn{2}{c}{\textbf{Pythia-6.9B}} & \multicolumn{2}{c}{\textbf{Pythia-12B}} & \multicolumn{2}{c}
    {\textbf{OPT-13B}} & \multicolumn{2}{c}{\textbf{NeoX-20B}} & \multicolumn{2}{c}{\textbf{Average}} \\
    \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14}  
    \textbf{Len.} & \textbf{Method} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} \\
    \midrule
    
    
    \multirow{8}{*}{32}
     & Loss \cite{yeom2018privacy} 
     & 61.4 & 61.6 & 63.8 & 64.1 & 65.5 & 65.6 & 62.6 & 62.4 & 68.8 & 68.3 & 64.4 & 64.4
     \\
     & Ref \cite{carlini2021extracting} 
     & 61.3 & 61.2 & 63.6 & 63.5 & 65.1 & 64.8 & \underline{65.9} & \textbf{65.5} & 67.3 & 66.2 & 64.6 & 64.2
     \\ 
     & Lowercase \cite{carlini2021extracting} 
     & 60.9 & 60.3 & 62.2 & 61.7 & 65.2 & 64.7 & 61.9 & 60.5 & 68.2 & 66.3 & 63.7 & 62.7
     \\ 
     & Zlib \cite{carlini2021extracting} 
     & 62.1 & 62.3 & 64.4 & 64.2 & 65.9 & 65.9 & 63.3 & 63.0 & 69.1 & 68.3 & 65.0 & 64.7
     \\ 
     & Min-K\% \cite{shi2023detecting} 
     & 61.8 & 61.7 & 66.3 & 65.2 & 68.2 & 67.1 & 64.0 & 63.2 & 71.6 & 69.7 & 66.4 & 65.4
     \\ 
     & Min-K\%++ \cite{zhang2024min}
     & 64.4 & 62.4 & 70.3 & 68.0 & \underline{73.2} & \underline{70.6} & \textbf{66.8} & \underline{64.4} & 75.2 & 70.1 & \underline{70.0} & 67.1
     \\ 
     & NormAR (ours)
     & \textbf{65.0} & \underline{63.4} & \textbf{70.6} & \underline{68.5} & \textbf{73.3} & \textbf{71.1} & 65.8 & 63.6 & \underline{75.8} & \underline{70.9} & \textbf{70.1} & \underline{67.5}
     \\
     & AR (ours)
     & \underline{64.6} & \textbf{63.8} & \underline{70.5} & \textbf{69.1} & 72.7 & \textbf{71.1} & 65.5 & 64.0 & \textbf{76.4} & \textbf{73.3} & 69.9 & \textbf{68.3}
     \\
    \midrule
    
    \multirow{8}{*}{64}
     & Loss \cite{yeom2018privacy} 
     & 58.4 & 56.5 & 60.7 & 59.3 & 61.8 & 59.9 & 58.7 & 57.1 & 66.4 & 63.8 & 61.2 & 59.3
     \\ 
     & Ref \cite{carlini2021extracting} 
     & 59.6 & \textbf{59.2} & 62.4 & 62.9 & 63.0 & 63.0 & 63.3 & \textbf{63.9} & 65.8 & 65.6 & 62.8 & 62.9
     \\ 
     & Lowercase \cite{carlini2021extracting} 
     & 57.8 & 56.1 & 58.2 & 57.7 & 59.5 & 59.0 & 58.6 & 57.2 & 65.6 & 64.0 & 59.9 & 58.8
     \\ 
     & Zlib \cite{carlini2021extracting} 
     & 60.6 & \underline{59.0} & 62.6 & 61.6 & 63.4 & 61.9 & 60.7 & 59.3 & 67.7 & 65.9 & 63.0 & 61.5
     \\  
     & Min-K\% \cite{shi2023detecting} 
     & 61.2 & 56.8 & 65.0 & 61.1 & 67.4 & 62.3 & 62.2 & 58.0 & 72.0 & 65.8 & 65.6 & 60.8
     \\ 
     & Min-K\%++ \cite{zhang2024min}
     & \textbf{65.0} & 58.5 & \textbf{71.6} & \underline{64.8} & \textbf{72.4} & \textbf{65.5} & \textbf{67.4} & \underline{59.9} & \underline{76.1} & 66.7 & \textbf{70.5} & 63.1
     \\  
     & NormAR (ours)
     & \underline{64.3} & \underline{59.0} & \underline{70.7} & \textbf{65.3} & \underline{70.8} & \underline{65.4} & \underline{65.5} & 59.7 & \textbf{76.3} & \underline{67.6} & \underline{69.5} & \textbf{63.4}
     \\
     & AR (ours)
     & 62.1 & 58.3 & 68.6 & 64.4 & 69.2 & 65.2 & 63.7 & 59.4 & 75.7 & \textbf{68.8} & 67.9 & \underline{63.2}
     \\
    \midrule
    
    \multirow{8}{*}{128} 
     & Loss \cite{yeom2018privacy} 
     & 62.8 & 62.3 & 65.1 & 64.7 & 65.6 & 65.4 & 63.2 & 62.4 & 70.2 & 69.3 & 65.4 & 64.8
     \\ 
     & Ref \cite{carlini2021extracting} 
     & 59.6 & 59.5 & 63.3 & 62.9 & 63.5 & 63.9 & 64.7 & 65.0 & 67.8 & 67.7 & 63.8 & 63.8
     \\ 
     & Lowercase \cite{carlini2021extracting} 
     & 59.5 & 59.6 & 60.5 & 60.0 & 60.6 & 60.4 & 59.5 & 58.6 & 66.8 & 66.7 & 61.4 & 61.1
     \\ 
     & Zlib \cite{carlini2021extracting} 
     & 65.0 & \underline{65.0} & 67.6 & \underline{67.4} & 67.7 & 68.1 & 65.1 & 65.1 & 71.9 & 71.7 & 67.5 & 67.5
     \\ 
     & Min-K\% \cite{shi2023detecting} 
     & 66.9 & 64.7 & 69.5 & 67.0 & 69.9 & 68.6 & 68.2 & 65.6 & 75.3 & \underline{72.4} & 70.0 & 67.7
     \\ 
     & Min-K\%++ \cite{zhang2024min}
     & 66.8 & 63.4 & \underline{70.7} & 66.8 & 71.8 & 68.9 & \underline{70.7} & 65.5 & \underline{76.3} & 71.6 & 71.3 & 67.2
     \\  
     & NormAR (ours)
     & \textbf{67.7} & \textbf{65.3} & \textbf{71.7} & \textbf{68.6} & \underline{72.1} & \textbf{70.3} & \textbf{72.1} & \textbf{67.8} & \underline{76.3} & \underline{72.4} & \textbf{72.0} & \textbf{68.9}
     \\
     & AR (ours)
     & \underline{67.4} & \underline{65.0} & \textbf{71.7} & \textbf{68.6} & \textbf{72.4} & \underline{69.9} & 69.6 & \underline{66.0} & \textbf{77.8} & \textbf{73.6} & \underline{71.8} & \underline{68.6}
     \\
    % \midrule
    % \multirow{8}{*}{256} 
    %  & Loss \cite{yeom2018privacy} 
    %  & 67.8 & - & 68.6 & - & 68.3 & - & 65.1 & - & 70.9 & - & 68.1 & -
    %  \\ 
    %  & Ref \cite{carlini2021extracting} 
    %  & 63.6 & - & 64.1 & - & 64.6 & - & \textbf{71.2} & - & 69.3 & - & 66.6 & -
    %  \\ 
    %  & Lowercase \cite{carlini2021extracting} 
    %  & 62.9 & - & 59.5 & - & 62.1 & - & 63.0 & - & 66.5 & - & 62.8 & -
    %  \\ 
    %  & Zlib \cite{carlini2021extracting} 
    %  & 69.3 & - & 69.8 & - & 70.8 & - & 67.4 & - & 72.8 & - & 70.0 & -
    %  \\ 
    %  & Min-K\% \cite{shi2023detecting} 
    %  & \underline{70.0} & - & \underline{71.7} & - & \underline{73.3} & - & 68.2 & - & \underline{76.7} & - & \underline{72.0} & -
    %  \\ 
    %  & Min-K\%++ \cite{zhang2024min}
    %  & 63.9 & - & 65.5 & - & 66.1 & - & 68.1 & - & 69.4 & - & 66.6 & -
    %  \\  
    %  & NormAR
    %  & 66.0 & - & 68.5 & - & 67.2 & - & \textbf{71.2} & - & 72.6 & - & 69.1 & -
    %  \\
    %  & AR
    %  & \textbf{70.1} & - & \textbf{72.6} & - & \undelrine{72.3} & - & \underline{70.9} & - & \textbf{77.2} & - & \textbf{72.6} & -
    %  \\
    \bottomrule
    \end{tabular}
    }
    \vspace{-0.4cm}
\end{table*}

==> tables_bold/wiki_tpr_results.tex <==
\begin{table*}[ht]
    \centering
    %\footnotesize
    \caption{TPR at low FPR (FPR=5\%) results on WikiMIA benchmark \protect\cite{shi2023detecting}. \textit{Ori.} and \textit{Para.} denote the original and paraphrased settings, respectively. \textbf{Bolded} and \underline{underlined} number shows the best result and the runner-up within each column across all methods.}
    \label{tab:wikimia_tpr}
    \resizebox{0.98\textwidth}{!}{%
    \begin{tabular}{llcccccccccccc}
    \toprule
    & & \multicolumn{2}{c}{\textbf{Pythia-2.8B}} & \multicolumn{2}{c}{\textbf{Pythia-6.9B}} & \multicolumn{2}{c}{\textbf{Pythia-12B}} & \multicolumn{2}{c}
    {\textbf{OPT-13B}} & \multicolumn{2}{c}{\textbf{NeoX-20B}} & \multicolumn{2}{c}{\textbf{Average}} \\
    \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14}  
    \textbf{Len.} & \textbf{Method} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} \\
    \midrule
    
    
    \multirow{8}{*}{32}
     & Loss \cite{yeom2018privacy} 
     & 14.7 & 14.2 & 14.2 & 15.0 & 18.1 & 16.3 & 11.9 & \underline{14.5} & 19.6 & 18.9 & 15.7 & 15.8
     \\
     & Ref \cite{carlini2021extracting} 
     & 6.2 & 7.2 & 6.7 & 6.2 & 9.8 & 8.8 & 9.3 & 8.3 & 16.3 & 14.2 & 9.7 & 8.9
     \\ 
     & Lowercase \cite{carlini2021extracting} 
     & 11.1 & 11.6 & 10.6 & 11.9 & 14.7 & 15.5 & 9.3 & 7.5 & 16.5 & 14.7 & 12.4 & 12.2
     \\ 
     & Zlib \cite{carlini2021extracting} 
     & 15.8 & \underline{14.5} & 16.3 & 12.7 & 17.6 & 15.0 & 13.7 & 13.4 & 19.4 & 17.3 & 16.6 & 14.6
     \\ 
     & Min-K\% \cite{shi2023detecting} 
     & \underline{17.1} & \textbf{16.5} & 17.8 & \textbf{21.7} & 20.9 & \underline{19.6} & \textbf{17.8} & 14.2 & \textbf{28.4} & 18.3 & \underline{20.4} & \underline{18.1}
     \\ 
     & Min-K\%++ \cite{zhang2024min}
     & 12.4 & 14.0 & 14.5 & 16.3 & 18.6 & 16.5 & 11.1 & 10.3 & 22.2 & 15.2 & 15.8 & 14.5
     \\ 
     & NormAR (ours)
     & \textbf{17.6} & 11.9 & \underline{18.1} & 15.0 & \textbf{21.7} & 17.3 & 8.0 & 12.4 & 24.5 & \underline{19.1} & 18.0 & 15.1
     \\
     & AR (ours)
     & 16.8 & 14.2 & \textbf{21.2} & \underline{17.8} & \textbf{24.0} & \textbf{24.3} & \underline{15.0} & \textbf{15.8} & \underline{26.4} & \textbf{23.8} & \textbf{20.7} & \textbf{19.2}
     \\
    \midrule
    
    \multirow{9}{*}{64}
     & Loss \cite{yeom2018privacy} 
     & 10.2 & 9.5 & 13.4 & 10.6 & 8.1 & 11.3 & 10.6 & 11.6 & 12.7 & 15.8 & 11.0 & 11.8
     \\ 
     & Ref \cite{carlini2021extracting} 
     & 10.6 & \underline{13.0} & 12.0 & \underline{16.2} & 11.6 & 15.5 & 8.8 & 9.5 & 14.4 & 15.5 & 11.5 & 13.9
     \\ 
     & Lowercase \cite{carlini2021extracting} 
     & 10.2 & 11.3 & 11.6 & 11.3 & 11.3 & 10.2 & 8.5 & 9.9 & 15.5 & 14.8 & 11.4 & 11.5
     \\ 
     & Zlib \cite{carlini2021extracting} 
     & 14.4 & \textbf{16.5} & 16.2 & 15.8 & 10.6 & 17.6 & 13.4 & \textbf{14.1} & 17.3 & \underline{19.0} & 14.4 & \textbf{16.6}
     \\ 
     & Min-K\% \cite{shi2023detecting} 
     & \underline{18.3} & 9.9 & 19.0 & 12.7 & \underline{23.6} & \underline{12.3} & \underline{17.3} & 11.3 & 21.8 & 13.7 & 20.0 & 12.0
     \\ 
     & Min-K\%++ \cite{zhang2024min}
     & 12.7 & 8.1 & 16.2 & 12.7 & 18.0 & \textbf{13.4} & 16.9 & 7.0 & 24.6 & 12.3 & 17.7 & 10.7
     \\  
     & NormAR (ours)
     & \textbf{18.7} & 11.6 & \underline{27.1} & \textbf{20.4} & 20.4 & 12.0 & 16.5 & 9.2 & \underline{27.8} & 16.9 & \underline{22.1} & 14.0
     \\
     & AR (ours)
     & 17.6 & 12.7 & \textbf{27.5} & 13.7 & \textbf{25.7} & 12.0 & \textbf{19.0} & \underline{12.0} & \textbf{28.2} & \textbf{21.8} & \textbf{23.6} & \underline{14.4}
     \\
    \midrule
    
    \multirow{9}{*}{128} 
     & Loss \cite{yeom2018privacy} 
     & 9.4 & \underline{14.4} & 14.4 & 16.5 & 15.8 & 19.4 & 17.3 & 15.8 & 15.1 & 20.9 & 14.4 & 17.4
     \\ 
     & Ref \cite{carlini2021extracting} 
     & 10.1 & 7.2 & 13.7 & 8.6 & 10.1 & 5.8 & 12.9 & 12.2 & 15.8 & 18.0 & 12.5 & 10.4
     \\ 
     & Lowercase \cite{carlini2021extracting} 
     & 10.8 & 8.6 & 12.9 & 11.5 & 11.5 & 10.1 & 9.4 & 7.2 & 16.5 & 14.4 & 12.2 & 10.4
     \\ 
     & Zlib \cite{carlini2021extracting} 
     & \textbf{18.7} & \textbf{16.5} & \underline{20.9} & \textbf{20.9} & 24.5 & \underline{19.4} & \underline{20.9} & \textbf{18.7} & 22.3 & 21.6 & \underline{21.5} & \textbf{19.4}
     \\ 
     & Min-K\% \cite{shi2023detecting} 
     & 13.7 & 12.2 & 18.0 & 16.5 & 18.0 & 14.4 & 19.4 & 11.5 & \underline{26.6} & 18.7 & 19.1 & 14.7
     \\ 
     & Min-K\%++ \cite{zhang2024min}
     & 13.7 & 11.5 & 20.9 & 16.5 & \underline{26.6} & \textbf{20.9} & 18.0 & \underline{18.0} & 18.7 & 19.4 & 19.6 & 17.3
     \\  
     & NormAR (ours)
     & 14.4 & 12.2 & \textbf{22.3} & \underline{20.1} & \textbf{28.1} & \textbf{20.9} & 17.3 & 15.1 & 21.6 & \underline{23.0} & 20.7 & 18.3
     \\
     & AR (ours)
     & \underline{15.1} & 12.9 & 19.4 & 18.7 & 21.6 & 17.3 & \textbf{22.3} & 17.3 & \textbf{37.4} & \textbf{25.9} & \textbf{23.2} & \underline{18.4}
     \\
    % \midrule
    
    % \multirow{8}{*}{256} 
    %  & Loss \cite{yeom2018privacy} 
    %  & 3.9 & - & 5.9 & - & 5.9 & - & 9.8 & - & 13.7 & - & 7.8 & -
    %  \\ 
    %  & Ref \cite{carlini2021extracting} 
    %  & 3.9 & - & 5.9 & - & 5.9 & - & 3.9 & - & 2.0 & - & 4.3 & -
    %  \\ 
    %  & Lowercase \cite{carlini2021extracting} 
    %  & 2.0 & - & 3.9 & - & 7.8 & - & 9.8 & - & 3.9 & - & 5.5 & -
    %  \\ 
    %  & Zlib \cite{carlini2021extracting} 
    %  & \textbf{19.6} & - & \textbf{27.5} & - & \textbf{21.6} & - & 21.6 & - & \textbf{25.5} & - & \textbf{23.2} & -
    %  \\ 
    %  & Min-K\% \cite{shi2023detecting} 
    %  & \underline{7.8} & - & 13.7 & - & 11.8 & - & 11.8 & - & \underline{23.5} & - & 13.7 & -
    %  \\ 
    %  & Min-K\%++ \cite{zhang2024min}
    %  & 3.9 & - & 5.9 & - & 9.8 & - & \underline{25.5} & - & 9.8 & - & 11.0 & -
    %  \\  
    %  & NormAR
    %  & \textbf{19.6} & - & 17.6 & - & 7.8 & - & \textbf{31.4} & - & 11.8 & - & \underline{17.6} & -
    %  \\
    %  & AR
    %  & \underline{7.8} & - & \underline{19.6} & - & \underline{17.6} & - & 23.5 & - & 11.8 & - & 16.1 & -
    %  \\
    \bottomrule
    
    
    \end{tabular}
    }
    
    \end{table*}

==> tables_bold/wikimia_patent_auc.tex <==
\begin{table*}[t]
\centering
\small % font size
\setlength{\tabcolsep}{4.pt} % column separation
\renewcommand{\arraystretch}{1.1} % row space 
\begin{tabular}{l cccc cccccccccc}
\toprule
\multirow{4}{*}{\textbf{Method}} & \multicolumn{4}{c}{PatentMIA} & \multicolumn{10}{c}{WikiMIA}                
\\ 
\cmidrule(r){2-5}
\cmidrule(r){6-15} 
% \cmidrule{5-8} 
% & Baichuan-13B   & Qwen1.5-14B   & OPT-6.7B & Pythia-6.9B & Pythia-12B & OPT-13B & GPT-NeoX-20B
& \multirow{2}{*}{\textbf{B-13B}}  & 
\multirow{2}{*}{\textbf{B2-13B}}  & 
\multirow{2}{*}{\textbf{Q-32B}}   &
\multirow{2}{*}{\textbf{Q-72B}}   &
\multicolumn{2}{c}{\textbf{OPT-6.7B}} & \multicolumn{2}{c}{\textbf{Pythia-6.9B}} & \multicolumn{2}{c}{\textbf{Pythia-12B}} & \multicolumn{2}{c}{\textbf{OPT-13B}} & \multicolumn{2}{c}{\textbf{NeoX-20B}}
\\ 
\cmidrule(r){6-7}
\cmidrule(r){8-9}
\cmidrule(r){10-11}
\cmidrule(r){12-13}
\cmidrule(r){14-15}

& & & & & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.}
\\ 
\midrule
Loss
& 60.8 & 63.0 & 60.9 & 54.7
& 62.4    & 61.5    & 65.1    & 64.3    & 65.3    & 65.1    & 63.2    & 62.3    & 70.4    & 69.3
\\
Ref
& 60.4 & 47.4 & 57.6 & 34.2
& 63.6    & 63.7    & 61.8    & 59.8    & 62.2    & 60.6    & 64.8    & 65.0    & 68.0    & 67.7
\\
Lowercase
& - & - & - & -
& 58.4    & 57.4    & 59.9    & 59.1    & 60.4    & 60.0    & 59.3    & 58.7    & 66.8    & 66.7
\\
Zlib
& 63.6 & 67.6 & 63.6 & 53.5
& 64.3    & 64.3    & 67.3    & 67.0    & 67.5    & 67.7    & 65.2    & 65.1    & 72.0    & 71.8
\\
Min-K\%
& 66.7 & 70.1 & 67.5 & 59.1
& 67.4    & 64.7    & 69.1    & 66.9    & 69.8    & 67.8    & 68.1    & 65.5    & 75.5    & 72.3
\\
Min-K\%++
& 62.8 & 66.6 & 66.6 & 65.1
& 69.0    & 64.9    & 70.4    & 66.1    & 71.4    & 67.8    & 70.8    & 65.4    & 75.4    & 71.8
\\
DC-PDD
& 70.0 & 74.7 & 70.1 & 61.4
& 67.9    & 66.1    & 69.5    & 68.0    & 70.1    & 68.1    & 67.5    & 66.1    & 75.8    & 73.1
\\
\hline
AR
& 73.4 & 78.0 & 77.0 & 80.1
& 70.1    & 68.0    & 72.2    & 69.7    & 72.6    & 70.3    & 70.4    & 68.3    & 78.2    & 75.8
\\
Deravative
& 75.1 & 78.3 & \textbf{77.9} & \textbf{81.4}
& 70.2    & 68.1    & 72.3    & 69.8    & 72.6    & 70.3    & 70.5    & 68.4    & 78.2    & 75.9
\\
NormAR
& \textbf{76.5} & \textbf{78.5} & 77.7 & 80.8
& 71.4    & 70.6    & 73.5    & 70.5    & 74.1    & 71.3    & 73.3    & 69.8    & 78.1    & 74.9
\\
\bottomrule
\end{tabular}
\caption{AUC scores for detecting pretraining texts. \textbf{Bold} indicates the best performing method.}
\label{table2}
\end{table*}

==> tables_bold/wikimia_patent_tpr.tex <==
\begin{table*}[t]
\centering
\small % font size
\setlength{\tabcolsep}{4.pt} % column separation
\renewcommand{\arraystretch}{1.1} % row space 
\begin{tabular}{l ccc cccccccccc}
\toprule
\multirow{3}{*}{Method} & \multicolumn{3}{c}{PatentMIA} & \multicolumn{10}{c}{WikiMIA}                
\\ 
\cmidrule(r){2-4}
\cmidrule(r){5-14} 
% \cmidrule{5-8} 
% & Baichuan-13B   & Qwen1.5-14B   & OPT-6.7B & Pythia-6.9B & Pythia-12B & OPT-13B & GPT-NeoX-20B
& \multirow{2}{*}{\textbf{Baichuan-13B}}  & 
\multirow{2}{*}{\textbf{Baichuan2-13B}}  & 
\multirow{2}{*}{\textbf{Qwen1.5-14B}}   & \multicolumn{2}{c}{\textbf{OPT-6.7B}} & \multicolumn{2}{c}{\textbf{Pythia-6.9B}} & \multicolumn{2}{c}{\textbf{Pythia-12B}} & \multicolumn{2}{c}{\textbf{OPT-13B}} & \multicolumn{2}{c}{\textbf{NeoX-20B}}
\\ 
\cmidrule(r){5-6}
\cmidrule(r){7-8}
\cmidrule(r){9-10}
\cmidrule(r){11-12}
\cmidrule(r){13-14}

 & & & & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.}
\\ 
\midrule
Loss
& 16.3    & 18.6    & 16.1
& 12.9    & 15.1    & 15.1    & 15.8    & 15.8    & 18.7    & 17.3    & 15.8    & 20.1    & 18.0
\\
Ref
& 14.0    & 3.4    & 4.4
& 10.8    & 8.6    & 16.5    & 10.8    & 9.4    & 10.1    & 12.9    & 12.9    & 15.8    & 18.7
\\
Lowercase
& -    & -    & -
& 10.1    & 7.9    & 12.9    & 12.2    & 13.7    & 11.5    & 8.6    & 7.9    & 12.9    & 12.9
\\
Zlib
& 16.1    & 16.8    & 13.0
& 18.0    & 15.1    & 20.1    & 19.4    & 23.7    & 19.4    & 20.9    & 18.7    & 21.6    & 22.3
\\
Min-K\%
& 17.3    & 21.7    & 16.8
& 20.9    & 15.8    & 18.7    & 19.4    & 23.7    & 20.9    & 19.4    & 18.7    & 24.5    & 22.3
\\
Min-K\%++
& 13.6    & 17.0    & 14.4
& 23.7    & 21.6    & 21.6    & 21.6    & 23.0    & 22.3    & 19.4    & 15.8    & 24.5    & 18.7
\\
DC-PDD
& 28.0    & 27.4    & 27.4
& 19.4    & 21.6    & 22.3    & 25.9    & 25.9    & 21.6    & 23.7    & 26.6    & 30.2    & 28.1
\\
\hline
AR
& 23.8    & 25.8    & 24.4
& 33.1    & 30.9    & 24.5    & 27.3    & 27.3    & 26.6    & 25.9    & 32.4    & 30.2    & 27.3
\\
Deravative
& 25.9    & 25.2    & 25.4
& 33.1    & 30.9    & 24.5    & 26.6    & 27.3    & 26.6    & 26.6    & 30.2    & 28.8    & 27.3
\\
NormAR
& 26.3    & 24.3    & 21.0
& 30.2    & 35.3    & 24.5    & 25.2    & 28.8    & 26.6    & 22.3    & 29.5    & 28.1    & 25.2
\\
\bottomrule
\end{tabular}
\caption{TPR for 5\%FPR scores for detecting pretraining texts. \textbf{Bold} indicates the best performing method.}
\label{table2}
\end{table*}
